Twisted chiral algebras of class $\mathcal{S}$ and mixed Feigin-Frenkel gluing

The correspondence between four-dimensional $\mathcal{N}=2$ superconformal field theories and vertex operator algebras, when applied to theories of class $\mathcal{S}$, leads to a rich family of VOAs that have been given the monicker chiral algebras of class $\mathcal{S}$. A remarkably uniform construction of these vertex operator algebras has been put forward by Tomoyuki Arakawa in arXiv:1811.01577. The construction of arXiv:1811.01577 takes as input a choice of simple Lie algebra $\mathfrak{g}$, and applies equally well regardless of whether $\mathfrak{g}$ is simply laced or not. In the non-simply laced case, however, the resulting VOAs do not correspond in any clear way to known four-dimensional theories. On the other hand, the standard realisation of class $\mathcal S$ theories involving non-simply laced symmetry algebras requires the inclusion of outer automorphism twist lines, and this requires a further development of the approach of arXiv:1811.01577. In this paper, we give an account of those further developments and propose definitions of most chiral algebras of class $\mathcal S$ with outer automorphism twist lines. We show that our definition passes some consistency checks and point out some important open problems.

==> sections/sec_4_twisted_fixtures_mixed_gluing__with_commented_out_parts_.tex <==
%!TEX Root = ../main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{\label{sec:fixtures}Twisted trinions from mixed Feigin--Frenkel gluing}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Arakawa's construction is universal and is well defined for any semisimple $\gf$---including non simply laced Lie algebras.\footnote{The same is true for the putative construction of Moore--Tachikawa symplectic varieties in \cite{Ginzburg:2018}.} At the same time, there is no construction for vertex algebras that have both $\gf_u$ and $\gf_t$ symmetries (both twisted and untwisted punctures). A calculation comparing the character of~\cite{Arakawa:2018egx} and the index of~\cite{Lemos:2012ph} shows that the two vertex algebras cannot be isomorphic; we show this in Appendix~\ref{app:rewriting_characters}. There are some notable exceptions; namely, the index of the twisted cylinder and the character of $\D_{G_t}$ agree. Consequently, so must the index of the twisted cap and the character of $\W_{G_t}$.\footnote{Strictly speaking, the characters of the cylinder and cap VOAs don't exist due to infinite-dimensional weight spaces. However, one can proceed formally by working term-by-term in the sum over integral dominant weights; this can be understood from a vertex algebra perspective as considering the decomposition into blocks belonging to $\KL^\lambda$ for each $\lambda\in P^+$.} This suggests that $\D_{G_t}$ and $\W_{G_t}$ will be key building blocks for our construction; indeed, the algebras associated to the sphere with two maximal twisted punctures and one maximal/one minimal twisted puncture should be identified with $\D_{G_t}$ and $\W_{G_t}$, respectively.

In this section, we posit a construction for more general genus zero mixed vertex algebras. Our proposal takes advantage of Feigin--Frenkel gluing to define the mixed trinion with one untwisted and two twisted punctures. From this, in principle, all other genus zero vertex algebras can be constructed. Recalling our discussion of residual gauge symmetries in Section~\ref{ssec:twisted_background/HL}, we have some expectations regarding the behaviour of these mixed vertex algebras under gauging. In particular, unlike the untwisted case, we expect that the BRST cohomology of the \emph{untwisted} gauging of two such vertex algebras will not be concentrated in degree zero, but will rather enjoy some derived enhancement.

To establish such properties regarding untwisted and twisted gauging, we need to examine the decomposition of the mixed vertex algebras into semijective objects in both twisted and untwisted $\KL$ categories. This will be depend in a crucial way on the structure of critical-level Weyl modules over $\hat\gf_{t,\kappa_c}$ as modules over the untwisted Feigin--Frenkel centre $\zf(\gf_u)$. This will lead us to a technical interlude involving opers.

In the bulk of this section we assume that we are dealing with $\IZ_2$ twists. We return to the case of $\IZ_3$ twists near the end of the section.

% Hereafter, we shall use the subscripts $u$ and $t$ to distinguish between the various objects associated to $\gf_u$ and $\gf_t$. For example, $\KL_t$ is the Kazhdan--Lusztig category associated to $\hat{\gf}_{t,\kappa_c}$ and $\D_u$ are the chiral differential operators over $G_u$. We also restrict our attention to the $\IZ_2$ twist and leave the $\IZ_3$ case for the end.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\label{subsec:twisted_untwisted_FF}The (un)twisted Feigin--Frenkel centre and the mixed trinion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The mixed vertex algebras should simultaneously be vertex algebra objects in $\KL_u$ and in $\KL_t$, so they will admit actions of both Feigin--Frenkel centres. The construction of $\V_{G,s}$ suggests that the action of these Feigin--Frenkel centres should be identified, but of course the twisted and untwisted centres are not isomorphic. It will be useful, therefore, to first examine how the actions of these two Feigin--Frenkel centres interact with each other.

Let $\sigma\in\mathrm{Out}(\gf_u)$ be an outer automorphism, $\gf_u^\sigma$ be the $\sigma$-invariant subalgebra of $\gf_u$, and $\gf_t = \left( \gf_u^\sigma \right)^\vee$. There exists a projection~\cite{Fuchs1996},
%%%%%%
\begin{equation}
	\pi_\sigma:\mathfrak{h}_u\twoheadrightarrow \mathfrak{h}_t~,
\end{equation}
%%%%%%
from the Cartan subalgebra of $\gf_u$ to that of $\gf_t$ that projects to elements that are invariant under $\sigma$. The outer automorphism lifts to an automorphism of $U(\gf_u)$ and we have a surjection
%%%%%%
\begin{equation}
	Z(U(\gf_u))\twoheadrightarrow Z(U(\gf_t))~,
\end{equation}
%%%%%%
which is just the projection of the centre of $U(\gf_u)$ to its $\langle \sigma\rangle$-coinvariants,~\ie, we set the $\sigma$-non-invariant generators of $Z(\gf_u)$ to zero. The action of $\sigma$ can be lifted to $\hat{\gf}_{u,\kappa_c}$ according to $\sigma(xt^n)=\sigma(x)t^n$. This gives a projection
%%%%%%
\begin{equation}\label{eq:FF_projection}
	\ZZ_u \twoheadrightarrow \ZZ_t\cong (\ZZ_u)_\sigma~,
\end{equation}
%%%%%%
where $(\ZZ_u)_\sigma$ is the space of $\langle\sigma\rangle$-coinvariants of the untwisted Feigin--Frenkel centre. 

The projection $\pi_\sigma$ also induces an embedding of weight spaces
%%%%%%
\begin{equation}
	\iota: P^+_t \hookrightarrow P^+_u~,
\end{equation}
%%%%%%
with image $\iota(P_t^+)$ equal to the subset of elements in $P^+_u$ that are invariant under the action of $\sigma$. For example if $\gf_u=D_n$ and $\gf_t=C_{n-1}$ (so $\sigma$ is the generator of the $\IZ_2$ outer automorphism), we have
%%%%%%
\begin{equation}
	\iota(\lambda_1,\lambda_2,\dots,\lambda_{n-1}) = (\lambda_1,\lambda_2,\dots,\lambda_{n-1},\lambda_{n-1})~.
\end{equation}
%%%%%%
In~\cite{Lemos:2012ph}, this was indicated with the notation $\lambda'=\lambda$. We will abuse notation and use $\lambda$ for both the weight in $P_t^+$ and its image  under $\iota:P_t^+\hookrightarrow P_u^+$. So $V_\lambda^t$ denotes the finite dimensional irreducible representation of $\gf_t$ with highest weight $\lambda$, and $V^u_{\lambda}$ is the finite dimensional irreducible representation of $\gf_u$ with highest weight $\iota(\lambda)$.

%Include Distler new here.. the projection depends on $\sigma$ etc.

Given an object $M\in\ZZ_t$-Mod, we can lift it to a module in $\ZZ_u$-Mod via the restriction of scalars associated to $\ZZ_u\twoheadrightarrow \ZZ_t$, giving a functor $\ZZ_t\text{-Mod}\rightarrow\ZZ_u\text{-Mod}$. The mixed vertex algebras must simultaneously be objects in the $\KL$ categories of $\gf_u$ and $\gf_t$. In the case where there are no untwisted punctures, the algebra must still have a $\ZZ_u$-Mod structure. This is because any such algebra can be obtained via DS reduction of a vertex algebra object in $\KL_u$, and the DS reduction functor lands in $\ZZ_u$-Mod. 

The first mixed object we would like to construct is the vertex algebra corresponding to $\CC_{0,1,1}$, which has two $\KL_t$ actions and one $\KL_u$ action. The most natural guess for a construction of this algebra would be to FF glue an untiwsted cap ($\W_u$) to the twisted cylinder ($\D_t$) via the untwisted Feigin--Frenkel centre. The preceeding discussion assures us that $\D_t$ can be lifted from $\ZZ_t$-Mod to $\ZZ_u$-Mod, and as such we propose that the mixed trinion associated to $\CC_{0,1,1}$ is 
%%%%%%
\begin{equation}
	V_{1,1}\coloneqq\Hi{0}(\ZZ_u,\W_u\otimes\D_t)~.
\end{equation}
%%%%%%
This mixed trinion is the most important vertex algebra of our construction. Indeed, it is the basic building block of the TQFT along with the untwisted trinion $\V_{G_u,3}$. Before proceeding to more general surfaces, it will be useful to establish the key properties of $\V_{1,1}$.

The genus zero vertex algebras, $\V_{G,s}$ have filtrations whose succesive quotients are $\IV_{\lambda,s}$ or $D(\IV_{\lambda,s})$, for some integral dominant $\lambda$. This is key in establishing that $\V_{G,s}$ are semijective in $\KL_u$, which in turn implies that gauging is concentrated in degree zero due to Theorem~\ref{thm:gauge-van}. Such a filtration would be extremely useful in establishing the properties of $\V_{1,1}$ under the various types of gluing.

Ideally, in the mixed case the successive quotients would simultaneously be objects in $\KL_u$ and $\KL_t$, and the natural proposal for such an object would be of the form
%%%%%%
\begin{equation}
	\IV_{\lambda'}^u\otimes_{\zf^u_{\lambda'}}\IV_{\lambda}^t
\end{equation}
%%%%%%
where $\lambda\in P_t^+$ and $\lambda'\in P_u^+$. While it is obvious that $\ZZ_t$ modules can be lifted to $\ZZ_u$ modules by way of the projection $\ZZ_u\twoheadrightarrow \ZZ_t$, it is not so obvious that this should hold for the quotient modules $\zf^u_{\lambda'}$, which are more complicated. Furthermore, there is a question of how $\lambda$ and $\lambda'$ are related. Altogether, there is room for doubt over whether the suggested tensor product over $\zf^u_{\lambda'}$ is even well-defined. To show that such a lift does indeed exist---and that the tensor product is well defined---for special values of $\lambda'$, we will work in the language of opers.

\begin{table}
	\centering
	\input{./figs/FF-gens.tex}
	\caption{\label{tab:FF-twists}The monomial generators of the Feigin--Frenkel centres of the untwisted algebra $\gf_u$ and its associated twisted algebra $\gf_t$. Note that algebras of type $\df_n$ have two generators of degree $n$, only one of which is invariant under the outer automorphism. For the $\df_4$ case, neither generator of degree four is invariant under the $\IZ_3$ outer automorphism.}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\label{subsec:opers_and_FF}Opers and the Feigin--Frenkel centre}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This subsection is largely self-contained and may be skipped over by the reader who is less in these technical details. At the end of this subsection, we formulate a theorem in the language of opers that implies a lifting of $\zf_{t,\lambda}$ modules to $\zf_{u,\lambda'}$ modules. In the following subsection we will move on to investigate the properties of $\V_{1,1}$.

We will not require the full machinery of opers (as can be defined on general algebraic curves), but instead will proceed with only a selective review of opers on the (punctured) disk with a choice of local coordinate. For more details, we direct the reader to~\cite{Frenkel:2004,Frenkel:2007}.

Let $D=\mathrm{Spec}\, \IC[\![t]\!]$ be the formal disc and $D^\times=\mathrm{Spec}\, \IC(\!(t)\!)$ be the formal punctured disc. Let $G$ be a semisimple algebraic Lie group with $Lie(G)=\gf$, and $B\subset G$ a Borel subgroup of $G$ with $Lie(B)=\mathfrak{b}$. A $G$-oper on $D$ is the triple,
%%%%%%
\begin{equation}
	(\mathscr{F},\nabla,\mathscr{F}_B)~,
\end{equation}
%%%%%%
where $\mathscr{F}$ is a principal $G$-bundle on $D$, $\nabla$ is a $G$-connection on $\mathscr{F}$, and $\mathscr{F}_B$ is a reduction of $\mathscr{F}$ to the Borel subgroup $B$ such that $\mathscr{F}_B$ is transversal to $\nabla$. A $G$-oper on $D^\times$ is defined analogously.

The space of opers on the disc can be made more concrete as follows. Let $\Lambda_p(h)$ be the image of the Cartan generator of $\mathfrak{sl}_2$ under the principal embedding, $\Lambda_{p}:\mathfrak{sl}_2\rightarrow \gf$. This defines gradings
%%%%%%
\begin{equation}
	\gf = \bigoplus_{i} \gf_i~,\quad \mathfrak{b} = \bigoplus_i\mathfrak{b}_i~,
\end{equation}
%%%%%%
on $\gf$ and $\mathfrak{b}$ by eigenvalues of $\mathrm{ad}\, \Lambda_p(h)$. Let $p_{-1} = \Lambda_p(f)$ be the image of the $\mathfrak{sl}_2$ lowering operator and let $p_1=\Lambda_p(e)$ be the image of the raising operator. We define $V^{can}$ to be the subspace of $\mathfrak{n}= \bigoplus_{i>0}\mathfrak{b}_1$ that is invariant under $p_1$, \ie, it is the subspace spanned by highest weight vectors with respect to the embedded $\mathfrak{sl}_2$. The subspace has the decomposition
%%%%%%
\begin{equation}
	V^{can} = \bigoplus_{d_i} V_{d_i}^{can}~,
\end{equation}
%%%%%%
where $d_i$ are the exponents of $\gf$. Let $\{p_i\}$ be a basis of $V^{can}$ such that $p_i\in V^{can}_{d_i}$.\footnote{In the case of $D_{2n}$, the subspace $V^{can}_{2n}$ is two dimensional and we have two linearly independent vectors $p_{2n}$ and $\tilde{p}_{2n}$.} There is a clear similarity to the generators of $\zf(\gf)$.

We denote the space of all such $G$-opers on the $D$ and $D^\times$ by $\mathrm{Op}_{G}\, D$ and  $\mathrm{Op}_{G}\, D^\times$, respectively.
Let $t$ be a formal coordinate on $D$. By an appropriate gauge transformation~\cite{Frenkel:2007}, any $G$-oper can be put into the canonical form
%%%%%%
\begin{equation}
	\nabla = d + p_{-1} + \sum_{i=1}^{\mathrm{rk}\,\gf}v_i(t)p_i~,
\end{equation}
%%%%%%
where $v_i(t)\in\IC[[t]]$ or $v_i(t)\in\IC((t))$ for $D$ or $D^\times$, respectively. A celebrated theorem of Feigin and Frenkel~\cite{Feigin:1984} states that,
%%%%%%
\begin{equation}
	\zf(\gf) \cong \mathrm{Fun}( \mathrm{Op}_{^L G}\, D)~,
\end{equation}
%%%%%%
and
%%%%%%
\begin{equation}
	\ZZ \cong \mathrm{Fun}(\mathrm{Op}_{^L G}\, D^\times)~,
\end{equation}
%%%%%%
where $^L G$ is the Langlands dual group of $G$. %We work exclusively over $\IC$ and only concern ourselves with simple $\gf$, so we take $^L G$ to be the simply connected Lie group associated to the Lie algebra $\gf^\vee$. 
%{\bf CB: This can't be stated quite right; unless we've assumed something about the global form of $G$ already?}

The Feigin--Frenkel centre acts on the Weyl modules $\IV_\lambda$, and this action factors through a certain quotient of the algebra of functions on opers~\cite{Frenkel:2010}. Namely,
%%%%%%
\begin{equation}\label{eq:weyl-proj}
	\ZZ \xrightarrow{\sim} 	\mathrm{Fun}\,\mathrm{Op}_{^L G}(D^\times) \twoheadrightarrow\mathrm{Fun}\, \mathrm{Op}_{^L G}^{\lambda} \cong \mathrm{End}_{\hat{\gf}_{\kappa_c}}(\IV_\lambda)~.
\end{equation}
%%%%%%
The quotient arises as follows. The subscheme $\mathrm{Op}_{^L G} (D)^{\lambda, reg}\subset\mathrm{Op}_{^L G}(D)$ is that of opers on the disc with \emph{regular singularity, with residue $\lambda$, and with no monodromy}. (See~\cite{Frenkel:2007} for more details.) The subscheme $\mathrm{Op}_{^L G}^{\lambda}\subset \mathrm{Op}_{^L G}(D^\times)$ is the image of $\mathrm{Op}_{^L G} (D)^{\lambda, reg}$ under the natural inclusion
%%%%%%
\begin{equation}
	\mathrm{Op}_{^L G}(D)\hookrightarrow \mathrm{Op}_{^L G}(D^\times)~.
\end{equation}
%%%%%%
The kernel of the projection \eqref{eq:weyl-proj} onto the opers without monodromy is the annihilator ideal
%%%%%%
\begin{equation}
	I_\lambda= \mathrm{Ann}_{\zf}\IV_\lambda~.
\end{equation}
%%%%%%
Thus, we have
%%%%%
\begin{equation}
	\zf_\lambda \coloneqq \ZZ_{<0}/I_\lambda \cong \mathrm{Fun}\,\mathrm{Op}_{^L G}^{\lambda}~~,
\end{equation}
%%%%%
where $\zf_{\lambda}$ is the quotient we introduced in \eqref{eq:ff_quot}. 

The particulars of our case lead to some simplifications. We take $^LG_u$ to be the Langlands dual of the simply connected Lie group, $G_u$, with Lie algebra $\gf_u$. Since $\gf_u$ is simply laced , $\mathrm{Lie}(^LG_u)\cong\gf_u$. 

%Furthermore, $^L G_t = ^LG_u^\sigma$,~\ie the outer automorphism invariant subgroup of original untwisted Lie group. This will be the key ingredient in constructing our surjection.

From our discussion in Section~\ref{subsec:twisted_untwisted_FF}, we have the following projection
%%%%%%
\begin{equation}
	\mathrm{Fun\, Op}_{^LG_u}(D^\times)\twoheadrightarrow(\mathrm{Fun\, Op}_{^LG_u}(D^\times))_\sigma\cong \mathrm{Fun\, Op}_{^LG_t}(D^\times)~,
\end{equation}
%%%%%%
which gives a closed embedding of the schemes
%%%%%%
\begin{equation}
	\mathrm{Op}_{^LG_t}(D^\times)\cong(\mathrm{Op}_{^LG_u}(D^\times))^\sigma  \hookrightarrow \mathrm{Op}_{^LG_u}(D^\times)~,
\end{equation}
%%%%%%
where $(\mathrm{Op}_{^LG_u}(D^\times))^\sigma$ is the spectrum of $(\mathrm{Fun\, Op}_{^LG_u}(D^\times))_\sigma$.
This is nothing more than the surjection $\ZZ_u\twoheadrightarrow \ZZ_t$ of Section~\ref{subsec:twisted_untwisted_FF}, rephrased in the language of opers.

%Here the outer automorphism invariants on theto
%%%%%%%
%\begin{equation}
	%\mathrm{Op}_{G_u}^\sigma = \mathrm{Spec} ( (\mathrm{Fun\, Op}_{G_u})_\sigma)~,
%\end{equation}
%%%%%%%
%\ie, as the spectrum of the outer automorphism coinvariant functions.

%By realising the $^L G_t$-opers as this invariant subscheme, we have a natural surjection to the quotient
%%%%%%%
%\begin{equation}
 %\mathrm{Fun\, Op}_{G_u}(D^\times)\twoheadrightarrow \mathrm{Fun\, Op}_{G_u^\sigma}(D^\times)~,
%\end{equation}
%%%%%%
%and corresponding closed immersion
%%%%%%
%\begin{equation}
	%\mathrm{Op}_{G_u^\sigma}(D^\times) \hookrightarrow \mathrm{Op}_{G_u}(D^\times)~.
%\end{equation}
%%%%%%%

To restrict this surjection to the no-monodromy opers, it is necessary that $\lambda'$ be outer automorphism invariant, specifically $\lambda'=\iota(\lambda)$. We will continue to abuse notation and denote $\iota(\lambda)$ by $\lambda$. We then have the following.
%%%%%%
\begin{thm}\label{thm:closed_immersion}
The restriction of the closed immersion
%%%%%%
\begin{equation*}
	\mathrm{Op}_{ ^L G_t}(D^\times) \hookrightarrow\mathrm{Op}_{ ^L G_u}(D^\times)~.
\end{equation*}
%%%%%%
to the subscheme $\mathrm{Op}_{^L G_t}^{\lambda}$ factors as
%%%%%%
\begin{equation*}
	\mathrm{Op}_{^L G_t}^{\lambda}\hookrightarrow\mathrm{Op}_{^L G_u}^{\lambda}\hookrightarrow\mathrm{Op}_{ ^L G_u}(D^\times)~,
\end{equation*}
%%%%%%
with each map a closed immersion. Equivalently, the natural surjection
%%%%%%
\begin{equation*}
	\mathrm{Fun\, Op}_{^LG_u}(D^\times)\twoheadrightarrow (\mathrm{Fun\, Op}_{^LG_u}(D^\times))_\sigma~,
\end{equation*}
%%%%%%
restricts to a surjection
%%%%%%
\begin{equation*}
	\mathrm{Fun\, Op}^\lambda_{^LG_u}\twoheadrightarrow (\mathrm{Fun\, Op}^\lambda_{^LG_u})_\sigma~,
\end{equation*}
%%%%%%
on the quotient algebras.
\end{thm}
%%%%%%
This theorem is precisely the statement that there is a surjection $\zf^u_{\lambda}\twoheadrightarrow \zf^t_{\lambda}$.
We present a proof of this theorem utilising Miura opers and Cartan connections in Appendix~\ref{sec:proof_closed_immersion}. It will prove crucial in proving that our construction of mixed vertex algebras of class $\SS$ satisfy certain, desirable properties.

%\subsection{Mischenko-Fomenko Subalgebra and Gaudin Algebras}
%The projection $\ZZ_u\twoheadrightarrow \ZZ_t$ restricts to a projection $\zf_{u,\lambda}\twoheadrightarrow \zf_{t,\lambda}$, so long as the ideals satisfy
%\begin{equation}
%\label{eq:ideal_proj}
	%I_\lambda^u \subset \tilde{I}_\lambda^t~,
%\end{equation}
%where $\tilde{I}_\lambda^t$ is the kernel of the composition
%\begin{equation}
%\ZZ_{u,<0}\twoheadrightarrow \ZZ_{t,<0} \twoheadrightarrow \zf_{t,\lambda}~.
%\end{equation}
%The Weyl module $\IV_\lambda$ is free over the subalgebra
%\begin{equation}
	%\ZZ_{(<0)} = \IC[P_{i,(n)}\,| 1=1,\dots,\mathrm{rk}\,\gf\, n<0] \cong \IC[P_{i,n}\,|\, i=1,\dots,\mathrm{rk}\, \gf,\, n < -d_i -1]~,
%\end{equation}
%where $d_i$ is the $i$th exponent as before. The subscheme $\mathrm{Op}_{^L G_u}(D^\times)^{\lambda,reg}$ therefore looks like an infinite dimensional affine space. Indeed, there is an obvious projection
%\begin{equation}
	%\ZZ_{u,(<0)}\twoheadrightarrow \ZZ_{t,(<0)}~.
%\end{equation}
%The only possible obstruction for (\ref{eq:ideal_proj}) lies in the quotient $\zf_\lambda/\zf_{(<0)}$. Thus, we are done if we can find a projection,
%\begin{equation}
	%\zf_{u,\lambda}/\ZZ_{u,(<0)} \twoheadrightarrow \zf_{t,\lambda}/\zf_{t,(<0)}~,
%\end{equation}
%of algebras.

%Let $V_\lambda$ be the finite dimensional irreducible representation of $\gf$ with highest weight $\lambda$.
%We have the isomorphism~\cite{Arakawa:2018egx}
%\begin{equation}
	%\bar{\zf}_\lambda \coloneqq \zf_\lambda/\zf_{free} \cong V_{\lambda}~,
%\end{equation}
%The $\ZZ$ module $V_{\lambda}$ is cyclic~\cite{Feigin:2010}
%and has an algebraic structure inherited from the $\ZZ$ action.
%The $\ZZ$-Mod structure of $V_\lambda$ is through the surjection \begin{equation}
	%\zf \twoheadrightarrow \mathcal{A}_{f} ~,
%\end{equation}
%where $\mathcal{A}_f\subset U(\gf)$ is the Mischenko-Fomenko subalgebra and $f=p_{-1}$ is a principal nilpotent element in $\gf$. The Mischenko-Fomenko subalgebra is a free polynomial algebra over $\IC$ with $\frac{1}{2}(\dim\, \gf + \mathrm{rk}\, \gf)$ generators. As with the Feigin--Frenkel centre, we have the isomorphism~\cite{Feigin:2010}
%\begin{equation}
%\mathcal{A}_f \cong \mathrm{Fun}\, \mathrm{Op}_{ ^L G}(\mathbb{P})_{\varpi(-f)}~,
%\end{equation}
%that is $\mathcal{A}_f$ is isomorphic to the function on $^L G$ opers over the Riemann sphere with regular singularity at $0$ and $2$-residue $\varpi(-f)$ at $\infty$. Here $\varpi(-f)$ is the image of the nilpotent principal element in $^L \gf$.
%Concretely,
%\begin{equation}
	%\mathcal{A}_f = \IC[u_{j,n} | j=1,\dots, \mathrm{rk}\, \gf,\, n=0,\dots,d_j]~.
%\end{equation}
%The $\AA_f$ module, $V_\lambda$, is cyclic and so we have
%\begin{equation}
	%V_\lambda \cong \mathcal{A}_f/\mathrm{Ann}_{\mathcal{A}_f}\,V_\lambda
%\end{equation}
%Once more, we have the projection
%\begin{equation}
%\label{eq:misch_proj}
	%\mathcal{A}_{u,f}\twoheadrightarrow \mathcal{A}_{t,f}~,
%\end{equation}
%arising from $\ZZ_u\twoheadrightarrow \ZZ_t$.
%The constraint (\ref{eq:ideal_proj}) is, therefore, equivalent to requiring that the above projection restricts to a projection of the quotients:
%\begin{equation}
	%V^u_{\lambda} \twoheadrightarrow V^t_\lambda~.
%\end{equation}

%In~\cite{Feigin:2010}, it was shown that the annihilator ideal is generated by the subalgebra of $\mathrm{Fun}\, \mathrm{Op}_{^L G}(\mathbb{P})_{\varpi(-f)}$ with no monodromy about $0$. It was also shown that the generators of this no monodromy ideal form a regular sequence in $\mathcal{A}_f$ and its vanishing set is, therefore, zero dimensional with
%\begin{equation}
	%u_{j,n} = 0,\, u_{j,d_j} = C_j~,
%\end{equation}
%where $C_j$ is the value of the $(j+1)$th order Casimir operator on $V_\lambda$. The ring
%\begin{equation}
	%\bar{\mathcal{A}}_\lambda\coloneqq \mathcal{A}_f/\mathrm{Ann}_{\mathcal{A}_f}(V_\lambda)~,
%\end{equation}
%is local and Gorenstein with a single closed point corresponding to the value of $u_{j,n}$ above.

%We can, now, restate our claim in terms of polynomial rings with only finitely many indeterminates.
%There is a closed immersion
%\begin{equation}
%\label{eq:A_immersion}
	%\mathrm{Spec}\, \mathcal{A}_{t,f} \hookrightarrow \mathrm{Spec}\, \mathcal{A}_{u,f}
%\end{equation}
%resulting from the projection $\mathcal{A}_{u,f}\twoheadrightarrow \mathcal{A}_{t,f}$ by identifying common generators. We also have the closed immersion $\mathrm{Spec}\,\bar{\mathcal{A}}_{u,\lambda}\hookrightarrow \mathrm{Spec}\,\mathcal{A}_{u,f}$ from projecting to the quotient. With this our conjecture is as follows.

%\begin{conj}
%\label{conj:gaudin_immersion}
%When the closed immersion (\ref{eq:A_immersion}) is restricted to the closed subscheme $\mathrm{Spec}\, \bar{\mathcal{A}}_{t,\lambda}$ it factors as
%\begin{equation}\nonumber
	%\mathrm{Spec}\, \bar{\mathcal{A}}_{t,\lambda}\hookrightarrow\mathrm{Spec}\, \bar{\mathcal{A}}_{u,\lambda}\hookrightarrow\mathrm{Spec}\, \mathcal{A}_{u,f}~,
%\end{equation}
%with each morphism a closed immersion of schemes.
%\end{conj}

%Looking at the single closed point, we see that at generic values of $\lambda'$ such an embedding does not exist, since the closed points will not agree. There is a unique value of $\lambda'$ for a given $\lambda$ such that the closed point of $ \mathrm{Spec}\, \bar{\mathcal{A}}_{t,\lambda}$ agrees with the closed point of $\mathrm{Spec}\, \bar{\mathcal{A}}_{u,\lambda'}$

%It is also necessary that $V^u_{\lambda'}$ is outer automorphism invariant. In such a representation, the Casimirs of $\gf_u$ that do not have a corresponding operator in $\gf_t$ act as zero. Indeed, this is precisely the representation with
%\begin{equation}
	%\lambda' = \iota(\lambda)~,
%\end{equation}
%as desired.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Properties of the mixed trinion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

First, we make use of our digression into opers to make the following, technical proposition.
\begin{prop}\label{prop:kl_u}
Let $N$ be a $\zf^t_\lambda$-module. Then $N$ is an object of $KL_{u,0}$,~\ie\ there exists some $M\in\KL_u$ such that 
$$
 N = H^0_{DS}(u,M)
$$
\end{prop}
\begin{proof}
We shall prove this by explicitly constructing an object in $\KL_u$ whose DS reduction is isomorphic to $N$ as an object of $\zf^t_\lambda$-mod.
From Theorem~\ref{thm:closed_immersion}, the $\zf^t_{\lambda}$ action can be lifted to an action of $\mathfrak{z}^u_{\lambda}$.

Let $\IV_\lambda^u$ be the Weyl module of $\hat{\gf}_{u,\kappa_c}$ with highest weight $\iota(\lambda)$. The tensor product,
$$
	\IV_\lambda^u\otimes_{\zf_\lambda^u} N~,
$$
is well-defined, where the $\zf_\lambda^u$ action on $N$ is from the lift. By construction, this is an object in $\KL_u$ --- with respect to the $\hat{\gf}_{u,\kappa_c}$ action on the untwisted Weyl module. Let us consider its DS reduction,
$$
	H^0_{DS}(u,\IV_\lambda^u\otimes_{\zf_\lambda^u} N)~.
$$
By way of the K\"unneth theorem, noting that $H^0_{DS}(\IV_\lambda)\cong\zf_\lambda^u$~\cite{Frenkel:2010} is obviously free over itself, we have that
$$
	H^0_{DS}(u,\IV_\lambda^u\otimes_{\zf_\lambda^u} N) \cong \zf^u_\lambda\otimes_{\zf_\lambda^u}N \cong N~,
$$
as desired.
\end{proof}
With this in hand we can establish an important theorem.

\begin{thm}\label{thm:cyl_kl0} 
We have the following isomorphism.
$$
H^0_{DS}(u,\V_{1,1}) \cong \D_t~,
$$
and so $\D_t \in \KL_{u,0}$.
\end{thm}
At the level of pictures, this theorem sounds almost trivial; if one starts with $\CC_{0,1,1}$ and closes the maximal untwisted puncture, the resulting surface is clearly the cylinder of type $\gf_t$. The proof of the above theorem, however, is not so straightforward, since $H^0_{DS}(u,\Hi{0}(\ZZ_u,\W_u\otimes -))$ is not necessarily the identity on a generic object in $\ZZ_u$-Mod. We leave the full proof of the this theorem to Appendix~\ref{app:proof_cyl} , instead we shall provide a sketch. 

The proof proceeds by first establishing that $\ch~ H^0_{DS}(u,\V_{1,1})_{\lambda} \le \ch~ \D_{t,[\lambda]}$,~\ie\ each weight space (with fixed generalised eigenvalue under the Harish-Chandra centre) of $H^0_{DS}(u,\V_{1,1})$ is smaller than that of $\D_t$. To do so we leverage the fact that $\D_t$ has an increasing filtration with subquotients $\IV^t_{\lambda,2}$, which, are in $\KL_{u,0}$ by by Proposition~\ref{prop:kl_u}. Since $\D_t$ is simple we need only construct a non-zero homomorphism $\D_t\rightarrow H^0_{DS}(u,\V_{1,1})$ to establish the isomorphism. To construct such a homomorphsim we adapt the proof of Theorem $9.9$ of~\cite{Arakawa:2018egx} to the twisted case.

This theorem shall serve as the foundation on which all the other properties of the genus zero mixed vertex algebras rest.

%\medskip

\begin{prop}\label{prop:trin_free_cofree}
The mixed trinion $\V_{1,1}$ is semijective in $\KL_t$.
\end{prop}
\begin{proof}
The cylinder $\D_t$ has an increasing filtration~\cite{frenkel2004}
$$
	0=N_0\subset N_1\subset N_2 \subset \dots ~,\quad N = \bigcup N_i \cong \D_t~,
$$
whose successive quotients
$$
	N_{i}/N_{i-1} \cong \IV_\lambda^t\otimes_{\zf^t_\lambda}\IV_{\lambda^*}^t~,
$$
for some $\lambda\in P_t^+$ and $\lambda^*$ the dual representation. Each $N_i/N_{i-1}$ is an object in $\zf_{\lambda}$ and so Proposition~\ref{prop:kl_u} applies and $N_i/N_{i-1}\in\KL_{u,0}$. Applying our Theorem~\ref{thm:cyl_kl0} and Theorem $9.14$ of~\cite{Arakawa:2018egx}, the mixed vertex algebra $\V_{1,1} \cong \W_u\ast_u \D_t$ has the increasing filtration
$$
	0= M_0\subset M_1 \subset M_2 \subset \dots ~,\quad M = \bigcup M_i \cong \V_{1,1}
$$
with successive quotients $M_i/M_{i-1}$ isomorphic to $\Hi{0}(\ZZ_u,\W_u\otimes N_{i}/N_{i+1})$. But from Proposition~\ref{prop:kl_u}, $N_i/N_{i-1}$ is in $\KL_{u,0}$ with $N_i/N_{i-1}\cong H^0_{DS}(u,\IV^u_\lambda\otimes_{\zf^u_{\lambda}}N_{i}/N_{i-1})$. Thus 
$$
	M_i/M_{i-1} \cong \IV_\lambda^u \otimes_{\zf^u_\lambda} \left( \IV^t_\lambda\otimes_{\zf^t_\lambda}\IV_{\lambda^*}^t \right)~.
$$
The action of  $U(t^{-1}\gf_t[t^{-1}])$ on either of the Weyl modules $\IV^t_{\lambda,\lambda^*}$ is projective and so $\V_{1,1}$ is projective over $U(t^{-1}\gf_t[t])$.
%The action of $U(t^{-1}\gf_u[t^{-1}])$ on $\IV^u_\lambda$, however, is not free since the tensor product over $\zf^u_\lambda$ means the action of any $\ZZ_u$ element that is not in $\ZZ_t$ is forced to be zero.
To establish that $\V_{1,1}$ is injective over $U(t\gf_t[t])$, we can repeat the same argument after taking $(\D_t)^{op}$ and noting that
$$
	(\D_t)^{op}\cong \D_t~.
$$
\end{proof}
Note that $\V_{1,1}$ is not semijective in $\KL_u$. To see this, consider the $\lambda=0$ terms in the filtration of $\V_{1,1}$, which form the affine current subalgebra of $\V_{1,1}$. Let $\ket{0}$ be the vacuum vector in $\IV_{0}^u$, any element $P_{i,-n}\ket{0}$ can be written as $\phi\ket{0}$ for a regular, $\phi\in U(t^{-1}\gf_u[t^{-1}])$. However, the modes $P_{i,-n}$, which are not invariant under $\sigma$, must act as zero on $\IV^u_{0}\otimes_{\zf_0^u}\IV^t_0\otimes_{\zf_0^t}\IV^t_0$. As there are regular elements in $U(t^{-1}\gf_u[t^{-1}])$ which act as zero, $\IV^u_{0}\otimes_{\zf_0^u}\IV^t_0\otimes_{\zf_0^t}\IV^t_0$ cannot be torsion free --- and so cannot be projective --- over $U(t^{-1}\gf_u[t^{-1}])$. 

The semijectivity of $\V_{1,1}$ in $\KL_t$ agrees with our beliefs on residual gauge symmetries. The surfaces $\CC_{0,m,1}$ formed by gluing $\CC_{0,1,1}$ along the twisted punctures have no residual gauge symmetry. Therefore the gluings $\V_{1,1}\circ_t-$ should be concentrated in cohomological degree zero, which we have just shown by arguing $\V_{1,1}$ is semijiective in $\KL_t$. On the other hand, gluing along the untwisted puncture should produce fermions, which falls in line with our argument that $\V_{1,1}$ is not semijectvie in $\KL_u$.

Having shown that $\V_{1,1}$ has the expected properties under $\circ_t$ and $\circ_u$, we move on to some more intrinsic properties of $\V_{1,1}$. Though our construction ensures that $\V_{1,1}$ is a vertex algebra, it is not at all clear that it has the properties expected from four-dimensional unitarity. Namely, $\V_{1,1}$ must be a conical, conformal vertex algebra with negative central charge. Let us first address the issue of the character.

\begin{prop}\label{prop:mixed_trin_char}
The character of the vertex algebra $\V_{1,1}$ is given by
$$
\mathrm{Tr}_{\V_{1,1}}(q^{L_0}\mathbf{a}\,\mathbf{b}_1\mathbf{b}_2) = \sum_{\lambda\in P_t^+} \frac{\KK_u(\mathbf{a})\chi^\lambda_u(\mathbf{a})\KK_t(\mathbf{b}_1)\chi_t^\lambda(\mathbf{b}_1)\KK_t(\mathbf{b}_2) \chi_t^\lambda(\mathbf{b}_2)}{\KK_u(\times)\chi_u^\lambda(\times)} ~,
$$
where $\mathbf{a}$ is a $G_u$ fugacity and $\mathbf{b}_i$ are $G_t$ fugacities. Furthermore, $\V_{1,1}$ is conical.
\end{prop}
\begin{proof}
By Theorem~\ref{thm:cyl_kl0}, we have that
$$
H^0_{DS}(u, \V_{1,1}) \cong \D_t~.
$$
As a graded vector space $\V_{1,1}\cong \bigoplus_{\lambda\in P_u^+} \V_{1,1\lambda}$, and by Proposition $8.4$ of~\cite{Arakawa:2018egx}.
$$
\mathrm{ch} \V_{1,1,\lambda} =  q^{\lambda(\rho^\vee)}\mathrm{ch}\, \mathbb{L}_\lambda \mathrm{ch}H^0_{DS}(u,\V_{1,1,\lambda})
$$
From the structure of the cylinder, we know that $H^0_{DS}(u,\V_{1,1,\lambda})$ is zero unless it is in the image of $\iota:P_t^+ \hookrightarrow P_u^+$. Therefore, we have 
$$
\mathrm{ch}\, \V_{1,1,\lambda} = q^{\lambda(\rho^\vee)}\mathrm{ch}\, \mathbb{L}^u_\lambda \mathrm{ch} \IV^t_\lambda \otimes_{\zf^t_\lambda}\IV_{\lambda*}^t~.
$$
Recalling Section~\ref{ssec:twisted_background/index} and the appendix of~\cite{Lemos:2014lua}, we can rewrite this in the notation of $\KK$-factors, giving the desired result.

To show that $\V_{1,1}$ is conical, note that the cylinder, $\D_t$, is non-negatively graded and
$\lambda(\rho^\vee)\ge0$ since it is integral dominant, with equality only for $\lambda=0$ --- establishing that $\V_{1,1}$ is non-negatively graded by weight. The character $\ch~ \V_{1,1,0}=1+\dots$ since $\IL_{\lambda=0}^u$ and $\D_{t,\lambda=0}$ are both conical. Thus the mixed trinion is conical.
\end{proof}


\begin{prop}\label{prop:mixed_trin_conf}
The vertex algebra $\V_{1,1}$ is conformal with central charge
$$
c_{\V_{1,1}} = 2\dim\,\gf_t + \dim \gf_u -\rk \gf_u  -24 \rho_u\cdot \rho_u^\vee~.
$$
\end{prop}
\begin{proof}
This proof relies on ideas from the proof of Proposition $10.7$ of~\cite{Arakawa:2018egx}.
The vertex algebras $\W_u$, $\D_t$ and the ghost system, $\Li{\bullet}(\zf(\gf_u))$ are all conformal, and we denote their respective conformal vectors by $\omega_\W$, $\omega_{\D}$ and $\omega_{gh}$.  Clearly, $\omega = \omega_\W+\omega_{\D}+\omega_{gh}$ is a conformal vector for the complex, $\W_u\otimes \D_t \otimes \Li{\bullet}(\zf(\gf_u))$. We write 
$$
\omega(z) = \sum_{m\in\IZ} L_m z^{-m-1}~,
$$
for the associated field.

By Lemma $9.4$ of~\cite{Arakawa:2018egx} the Feigin--Frenkel centre of $\W_u$ is preserved by the action of $L_m$ for $m\ge -1$. For a generator $P_i\in\zf(\gf_u)$,
$$
\omega(z) P_i(w) \sim \frac{\partial P_i}{z-w} +\frac{(d_i+1) P_i}{(z-w)^2}+\sum_{j=2}^{d_i+2}\frac{(-1)^j j!}{(z-w)^{j+1}} q_j^{(i)}(w)~,
$$
where $q_j^{(i)}$ is some homogeneous state in $\zf(\gf_u)$ with weight $d_i-j+2$. Let us denote by $\widetilde{P_i}$ the image of $P_i$ under the projection $\zf(\gf_u)\twoheadrightarrow \zf(\gf_t)$.
One then has
$$
\omega(z) \widetilde{P_i}(w) \sim \frac{\partial \widetilde{P_i}}{z-w} +\frac{(d_i+1) \widetilde{P_i}}{(z-w)^2}+\sum_{j=2}^{d_i+2}\frac{(-1)^j j!}{(z-w)^{j+1}} \widetilde{q_j}^{(i)}(w)~,
$$
where we think of $\widetilde{P_i}$ as a state in $\zf(\gf_t)\subset\D_t$. Let $Q(z)$ be the BRST differential for FF gluing, we have that 
$$
Q_{(0)}(z) \omega(w) = \sum_{i=1}^{\mathrm{rk}\,\gf}\sum_{j=2}^{d_i+1} \partial^j \big(\rho_\W(q_j^{(i)}) -\rho_{\D_t}(\tau(q_j^{(i)}))\big)c_i~,
$$
where $\rho_W:\zf(\gf_u)\hookrightarrow \W_u$ and $\rho_{\D_t}:\zf(\gf_u)\hookrightarrow \D_t$ denote the action of the untwisted Feigin-Frenkel centres on $\W_u$ and on $\D_t$ via the projection to $\zf(\gf_t)$. Unfortunately, $\omega$ does not descend to cohomology and so we must consider correction terms to construct a putative conformal vector in cohomology.

If the right hand side of the above equation equals $Q_{(0)}\chi$ for some state $\chi$, then $\widetilde{\omega} = \omega + \chi$ is $Q$-closed and defines a vector in $\V_{1,1}$. to show that such a $\chi$ exists, it is sufficient to show that $\widetilde{q_j}^{(i)}= \pi(q_j^{(i)})$.

The action of $L_m$ for $m\ge-1$ on $\zf(\gf_u)$ is given by the action of $\mathrm{Der}(\OO_D)$ on $\mathrm{Op}_{^LG_u}(D)$, which correspond to infinitesmal co-ordinate changes on the formal disc~\cite{Frenkel:2007}. We postpone the full argument to Appendix~\ref{sec:proof_closed_immersion} for brevity, but by \eqref{eq:der_od_comm} the action of $\mathrm{Der}(\OO_D)$ intertwines and  $\widetilde{q_j}^{(i)}= \pi(q_j^{(i)})$. Thus $\widetilde{\omega}\in \V_{1,1}$.

Now, we wish to show that $\widetilde{\omega}$ is a conformal vector. The vector $\chi$ can be written as 
$$
\chi = \sum_{i=1}^{\mathrm{rk}\, \gf_u}\sum_{j=2}^{d_i+2} \partial^j (\rho_{\W}\otimes \rho_{\D_t}\otimes \rho_{gh})(z_{ij})~,
$$
for some $z_{ij} \in \zf(\gf_u)\otimes\zf(\gf_u)\otimes \Li{0}(\zf(\gf_u))$. Therefore, $\widetilde{\omega}_{(i)}=\omega_{(i)}$ for $i=0,1$, and so the OPEs agree up to the quadratic pole. 
Since $\V_{1,1}$ is non-negatively graded by Proposition~\ref{prop:mixed_trin_char}, Lemma 3.1.2 of~\cite{Frenkel:2007} says that all we need to check is that $\widetilde{\omega}_{(3)}\widetilde{\omega}= c/2\ket{0}$ for some $c\in\IC$.,~\ie\ the quartic pole in the Virasoro--Virasoro OPE is a multiple of the identity. 

However, we know that $\V_{1,1}$ is conical from its character and so the only operator of dimension zero that can appear in the OPE is the identity. Thus, $\widetilde{\omega}$ is a conformal vector of $\V_{1,1}$.

Finally, we wish to show that $\widetilde{\omega}$ and $\omega$ have the same central charge in cohomology. Note that $\V_{1,1}=\sum_{\Delta\in\IN} \V_{1,1}^{\Delta}$ with $\dim\, \V_{1,1}^\Delta<\infty$ and is conical --- so $\V_{1,1}$ is of CFT type. As a result, Lemma 4.1 of~\cite{Moriwaki_2020} applies. Namely, for any $x\in \V_{1,1}$, if $\Delta(x)\ge 2$ and $x_{(0)}\widetilde{\omega}=0$ then $x \in \mathrm{im}_{\widetilde{\omega}_{(-1)}}(\V_{1,1})$.

Now suppose $\omega'$ was some other conformal vector in $\V_{1,1}$, such that $\omega'_{(1)}$ agrees with $\widetilde{\omega}_{(1)}$. Then, we have that $(\omega'-\widetilde{\omega})_{(0)}\widetilde{\omega}=0$ and so $\omega'-\widetilde{\omega} = \partial x$ for some $x\in\V_{1,1}$ with $\Delta=1$. Since $\widetilde{\omega}_{(i)}=\omega'_{(i)}$ for $i=0,1$, we must have that $\partial x_{(i=0,1)}=0$ and so $x$ is central in $\V_{1,1}^{\Delta=1}$. Repeating the argument with $(\omega-\widetilde{\omega})_{(1)}$ and using the Borcherds identities, leads us to conclude that $\partial x =0$ and so $\widetilde{\omega}$ is unique.

Under DS reduction, $H^0_{DS}(u,\V_{1,1})\cong \D_t$ and the image of $\widetilde{\omega}$ gives rise to a conformal vector in $\D_t$. By a similar argument as the preceeding, one can show that this is the unique conformal vector which agrees with the grading on $\D_t$, see the proof of Proposition $10.7$ in~\cite{Arakawa:2018egx}. The central charge of $\D_t$ is $c_{\D_t}=2\dim\,\gf_t$ and the central charge of the image of $\widetilde{\omega}$ is related to $c_{\V_{1,1}}$ by
$$
c_{\D_t} = c_{\V_{1,1}} +\rk\,\gf_u - \dim \gf_{u} +24 \rho_{u}\cdot\rho^\vee_{u} ~,
$$
under DS reduction.
\end{proof}
With these propositions in hand, we have shown that $\V_{1,1}$ obeys many of the desirable properties one would expect from the chiral algebra associated to $\CC_{0,1,1}$. Yet we have not explicitly tied this object to the construction of~\cite{Beem:2013sza}. One might, rightfully, wonder whether the object we have constructed actually is the mixed trinion of class $\SS$. 

\begin{prop}~\label{prop:mixed_unique}
The mixed trinion $\V_{1,1}$ is the unique vertex algebra object in $\KL_u$ such that 
$$
H^0_{DS}(u,\V_{1,1})\cong \D_t~.
$$
\end{prop}
\begin{proof}
This follows fairly easily from the fact that $\D_t$ is an object in $\KL_{u,0}$. Suppose $V\in\KL_u$ is a vertex algebra object such that $H^0_{DS}(u,V)\cong \D_t$ we must have that 
$V \cong \W_u\ast_u \D_t $, since $\W_u\ast_u(H^0_{DS}(u,-)-$ is the identity in $\KL_u$. However, $\V_{1,1}\coloneqq \W_u \ast_u \D_t$ and so $V\cong \V_{1,1}$.
\end{proof}

Suppose, $\widetilde{\V}_{1,1}$ is the vertex algebra associated to $\CC_{0,1,1}$, computed by the cohomological method of~\cite{Beem:2013sza}. This must be a vertex algebra object in $\KL_u$, since it has an action of $V^{\kappa_c}(\gf_u)$ coming from the untwisted puncture and inherits a suitable grading from the physical grading of superconformal quantum numbers.
Performing untwisted DS reduction on $\tilde{\V}_{1,1}$ must produce the cylinder $\CC_{0,1,1}$ which has corresponding vertex algebra $\D_t$
%
%
\footnote{If one is uncomfortable with invoking the vertex algebra of the cylinder, which has no corresponding physical SCFT, consider the following argument. The physical vertex algebra $\widetilde{\V}_{1,1}$ must satisfy $\widetilde{\V}_{1,1}\circ_t \widetilde{\V}_{1,1}$. Performing DS reduction, we must have $H^0_{DS}(u,\widetilde{\V}_{1,1}\circ_t\widetilde{\V}_{1,1})\cong \widetilde{\V}_{1,1}$. By means of a spectral sequence argument, which we shall elaborate on in the next subsection , one may rearrange the order of cohomologies to show $H^0_{DS}(u,\widetilde{\V}_{1,1})\circ_t \widetilde{\V}_{1,1}\cong\widetilde{\V}_{1,1}$, which implies that $H^0_{DS}(u,\widetilde{\V}_{1,1})=\D_t$.}.
%
%
Of course, Proposition~\ref{prop:mixed_unique} applies and so we have 
%%%%%%
\begin{equation}
	\widetilde{\V}_{1,1}\cong \W_u\ast_u \D_t \cong \V_{1,1}~.
\end{equation}
%%%%%%
Indeed, $\V_{1,1}$ is the unique, up to isomorphism, vertex algebra object in $\KL_u$ which satisfies $H^0_{DS}(u,\V_{1,1})\cong \D_t$. 
%Additionally, $\V_{G_u,3}$ has a similar uniqueness condition in $\KL_u$~\cite{Arakawa:2018egx}. 
%Since $\V_{1,1}$ and $\V_{G_u,3}$ are the buillding blocks of the mixed vertex algebras, this extends to a uniqueness result on all the $\V_{m,n}$, under the mild assumption that the gauging structure of class $\SS$ is inherited by the vertex algebras.

%Let us try to make a concrete link between our constructions and the physics.
%For the $D_n,C_{n-1}$ case we have an expectation that $\V_f\cong \SS\BB$, where $\SS\BB$ is the symplectic boson algebra --- with appropriate flavour symmetry. Trying to link the vertex algebra $\V_f$ to the physical chiral algebras arising from physics is hard --- there are intricate relations between generators of the cap algebra. The cylinder algebra is better understood and so we claim the following:
%\begin{conj}\label{conj:free_boson}
%For $\gf_u=D_n$ and $\gf_t=C_{n-1}$, we have the isomorphism
%\[ 	H^0_{DS}(u,\SS\BB) \cong H^0_{DS}(t,\D_t)\cong \W_t~.\]
%\end{conj}
%By construction, $\SS\BB$ is a vertex algebra object in $\KL_u$ and  $\W_t \in \KL_{u,0}$, from Proposition~\ref{prop:cyl_kl0}.
%Equivalences, reflect isomorphisms and so we have
%\begin{equation}
	%H^0_{DS}(u,\V_f)\cong H^0_{DS}(u,\SS\BB) \implies \V_f\cong\SS\BB
%\end{equation}
%where the isomorphism should be understood as an isomorphism between vertex algebra objects in $\KL_u$. The converse of this statement is also true, and so Conjecture~\ref{conj:free_boson} is equivalent to the statement that $\V_f\cong \SS\BB$ in the $D_n$ case. However it is much more tractable to verify Conjecture~\ref{conj:free_boson} than it is to verify $\V_f\cong\SS\BB$.

%Hereafter, we shall assume Conjecture~\ref{conj:free_boson} to be true, but much of our construction will not explicitly rely on it. We believe this is a fairly sensible assumption to make. Indeed, if Conjecture~\ref{conj:free_boson} is false, our entire construction --- while still being well-defined --- becomes rather futile since we would not be constructing the physical chiral algebras of Class $\SS$.

%The twisted case resists the cap gluing construction of the untwisted case. We are not able to define all twisted genus zero vertex algebras via FF-gluing of caps. This is largely due to the fact that the vertex algebras $\V_{\gf_t,s}$ defined via FF-gluing caps do not correspond to the vertex algebras of surfaces with twisted punctures for $s>2$. Indeed, we note that for $s>2$ there is residual gauge symmetry and we should expect the presence of fermions. These fermions cannot be introduced by applying $\Hi{0}(\ZZ_t,\W_t\otimes-)$ but a construction relying on gauging can reproduce these fermions. This is because the algebras, $\V_{m,n}$ are not semijective in $\KL_u$ and so the higher cohomologies of gauging are non-vanishing.

Thus far, we have been fairly abstract, but let us provide some concrete observations. We have argued that the mixed trinion $\V_{1,1}$, as we have constructed it, is the unique vertex algebra associated to $\CC_{0,1,1}$. Let us consider the vertex algebra associated to $\CC_{f}$, which is a genus zero surface with one maximal untwisted puncture, one maximal twisted puncture and an empty twisted puncture. The corresponding vertex algebra is $\V_{f}=H^0_{DS}(t,\V_{1,1})$.

The surface $\CC_f$ does correspond to a physical SCFT. When $\gf_u=\df_n$, $\gf_t=\mathfrak{c}_{n-1}$ and the corresponding SCFT is a free hypermultiplet theory, hence the subscript $f$. In this case $\V_f$ should be a symplectic boson vertex algebra with a commuting $\hat{\gf}_{u,\kappa_c}\times\hat{\gf}_{t,\kappa_c}$ subalgebra. Unfortunately, this does not hold for the other choices of $\gf_u$ (at generic rank). There is, however, another example that has appeared in recent literature. The even rank Lie algebras $\gf_u=\af_{2n}$ have,  as their  twisted algebras, $\gf_t=\mathfrak{c}_{n}$ --- unlike the $\df_n$ theories the SCFT has a global Witten anomaly. For $\gf_u=\af_2$ and $\gf_t=\mathfrak{c}_1=\af_1$, the SCFT is the $\TT_X$ theory of~\cite{Buican:2017fiq}, the class $\SS$ realisation was given in~\cite{Beem:2020pry}. The associated vertex algebra is given in~\cite{Buican:2017fiq}. In the $E_6$ and $A_{2n+1}$ cases, these vertex algebras remain somewhat mysterious.

It is also interesting to note that $\V_f$ should be conical, despite the fact that it is obtained from the FF gluing of two caps. In the cases where the two caps are of the same type, one obtains the cylinder $\D_u$ or $\D_t$ --- neither of which are conical.

Noticing that $\V_{f}$ is a symplectic boson system for $\gf_u=\mathfrak{d}_n$ leads to a curious observation. Take the symplectic boson system, $\SS\BB$ associated to the bifundamental representation of $\gf_u\times \gf_t$, its DS reduction must be isomorphic to the DS reduction of $\V_f$. This implies that for $\gf_u = \df_n$, 
%%%%%%
\begin{equation}\label{eq:ds_free}
	H^0_{DS}(u, \SS\BB) \cong H^0_{DS}(u,\V_f)\cong \W_t~.
\end{equation}
%%%%%%
Indeed, this presents an alternate construction for the equivariant affine $\WW$-algebra, $\W_{C_{n-1}}$. While we cannot explicitly show this isomorphism, we present some supporting evidence for the low rank case in Appendix~\ref{app:ds_free}.

We have provided a fairly comprehensive list of properties of the mixed trinion, which is the building block of the twisted chiral algebras of class $\SS$. We would like to extend the results we have found to the other genus zero, mixed vertex algebras. As we increase the number of twisted and untwisted punctures, we will naturally be forced to consider how the various types of gluing interact with each other. Therefore, it shall be useful to have a list of rearrangement lemmas that establish the extent to which the various gluings associate.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\label{ssec:duality/rearr}Rearrangment lemmas}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We establish a series of technical rearrangement lemmas concerning the interplay between the various cohomological operations we have defined thus far. 
The proofs of these lemmas, which are modifications of proofs of~\cite{Arakawa:2018egx}, rely heavily on the machinery of spectral sequences. The reader who is not interested in technical details may wish to skip this section. In the next we expand our construction to the vertex algebras associated to $\CC_{0,m,n}$.
%It should be noted that our lemmas here do not depend on the veracity of Conjecture~\ref{conj:free_boson} and are strictly independent of it.

Since we are interested in the interplay of gluings, we want to consider objects that have multiple, commuting  $\hat{\gf}_{\kappa_c}$ actions. If one wishes to be completely precise, one should decorate each $\circ$ with subscripts for the action that is being gauged. This would be somewhat cumbersome, especially when it is contextually clear which actions are involved in the gluing.

Instead, we will be overloading our notation for $\circ$ to distinguish between the various actions on an object. The rearrangement lemmas are only concerned with two such actions, for the sake of argument we call them the left and right actions. Suppose $U,V,W$ are in $\KL$, such that $V$ has two actions of $\hat{g}_{\kappa_c}$ and $V$ is in $\KL$ with respect to both actions. 
One should then interpret the symbol $U\circ(V\circ W)$ as the semi-infinite cohomology $\Hi{\bullet}(\hat{\gf}_{-\kappa_g},\gf,U\otimes\Hi{\bullet}(\hat{\gf}_{-\kappa_g},\gf,V\otimes W))$, where the diagonal action of $\hat{\gf}_{-\kappa_g}$ is with respect to the right $\hat{\gf}_{\kappa_c}$ action on $V$ and the sole $\hat{\gf}_{\kappa_c}$ action on $W$. Similarly, the diagonal action on $U\otimes \Hi{\bullet}(\hat{\gf}_{-\kappa_g},\gf,V\otimes W)$ is with respect to the sole $\hat{\gf}_{\kappa_c}$ action on $U$ and the $\hat{\gf}_{\kappa_c}$ action on $V\circ W$ induced by the left action on $V$.

For objects $U,V,W\in\ZZ$-Mod, we will denote the semi-infinite cohomology $\Hi{0}(\ZZ,U\otimes\Hi{0}(\ZZ,V\otimes W))$ by  $U\ast(V\ast W)$. Here one should take the diagonal action on $V\otimes W$ for the first cohomology and on $U\otimes V$ for the second.

Hereafter, it should be understood that when one has many $\KL_u$, or $\KL_t$ actions we choose two such actions for the purposes of the rearrangement lemmas. For the chiral algebras of class $\SS$ (both untwisted and twisted), all the moment maps (from the same algebra) are symmetric and one can make such a choice without loss of generality. We will not pursue this notational issue further and hope that any ambiguities are resolved by context.

First, we shall shall recast some of the results of~\cite{Arakawa:2018egx} as rearrangement lemmas.

%%%%%%
\begin{lem}\label{lem:rearr_gauge}
Let $U,V,W$ be vertex algebra objects in $\KL$ such that $U$ is semijective in $\KL$ and $V$ has two $\KL$ actions, then
$$
U\circ(V\circ W)\cong (U\circ V)\circ W~.
$$
\end{lem}
\begin{proof}
%%%%%%
This proof is similar to the proof of Theorem 10.11 of~\cite{Arakawa:2018egx}.
Consider the bicomplex 
$$
C^{\bullet\bullet}= U\otimes V\otimes W\otimes \Li{\bullet}(\gf)\otimes\Li{\bullet}(\gf)~,
$$
with the differential $d_1$ acting on $U\otimes V$ and the first  $\Li{\bullet}(\gf)$ and $d_2$ acting on $V\otimes W$ and the second $\Li{\bullet}(\gf)$. It is easy to see that $d_1d_2+d_2d_1=0$ and so the total complex $C_{tot}^p = \bigoplus_{m+n=p}C^{m,n}$ is a cochain complex with the differential $d = d_1 + (-1)^m d_2$~\cite{Weibel:1994}. There are two spectral sequences converging to the total cohomology of $(C_{tot},d)$
\begin{equation}\nonumber
\begin{split}
	_IE^{p,q}_2 = \Hi{p}(\hat{\gf}_{-\kappa_g},\gf,U\otimes\Hi{q}(\hat{\gf}_{-\kappa_g},\gf,V\otimes W))~,\\
	_{II}E^{p,q}_2 = \Hi{p}(\hat{\gf}_{-\kappa_g},\gf,W\otimes\Hi{q}(\hat{\gf}_{-\kappa_g},\gf,U\otimes V))~.
\end{split}
\end{equation}

By Theorem \ref{thm:gauge-van}, the cohomologies $\Hi{p}(\hat{\gf}_{-\kappa_g},\gf,U\otimes-)$ are concentrated in degree zero and so both spectral sequences collapse at the second page. The only nonzero entries are $_I E_2^{0,q}$ and $_{II}E_2^{p,0}$. Thus, we have
$$
_IE^{0,p}_2\cong\ _{II}E^{p,0}_2 \cong H^p_{tot}(C_{tot},d)~,
$$
which gives the desired isomorphism.
\end{proof}

The vertex algebra objects $\V_{G,s}$ are semijective in $\KL$ and so composition of vertex algebras is associative --- in the untwisted setting. Furthermore, all gaugings at genus zero are concentrated in degree zero. In the twisted setting, we wil have to work harder.

%The vertex algebras $\V_{m,n}$ are not semijective in $\KL_u$ and our spectral sequence argument no longer holds generically. In fact we should expect the cohomology to no longer be concentrated in degree zero  since we believe that the Higgs branch of these theories has residual gauge symmetry for $n>2$. The gluing operation is, therefore, sensitive to whether the Higgs and HL chiral rings coincide or not.


We have a similar result for FF-gluing,
\begin{lem}\label{lem:rearr_ff}
Suppose $M_1,M_2,M_3\in\ZZ$-Mod and suppose that $M_1$ and $M_3$ are free over $\ZZ_{(<0)}$. 
Then
$$ M_1\ast (M_2\ast M_3)\cong (M_1\ast M_2)\ast M_3~.$$
\end{lem}
\begin{proof}
This proof is similar to the proof of Proposition 10.2 of~\cite{Arakawa:2018egx}.
Consider the bicomplex
$$
C^{\bullet\bullet} = M_1\otimes M_2\otimes M_3 \otimes \Li{\bullet}(\mathfrak{z}(\gf))\otimes\Li{\bullet}(\mathfrak{z}(g))~,
$$
with differentials $d_{12}$ acting on $M_1\otimes M_2 \otimes \Li{\bullet}(\mathfrak{z}(\gf))$ and $d_{23}$ acting on $M_2\otimes M_3\otimes \Li{\bullet}(\mathfrak{z}(\gf))$. The two differentials anticommute and so we can form the total complex $C_{tot}^n = \bigoplus_{p+q=n}C^{p,q}$ with total differential $d_{tot} = d_{12}+(-1)^q d_{23}$. There are two spectral sequences converging to the total cohomology $H_{tot}$ of $C_{tot}$, whose second pages are given by
\begin{equation}\nonumber
\begin{split}
_I E_2^{p,q} \coloneqq \Hi{p}(\ZZ,M_1\otimes\Hi{q}(\ZZ,M_2\otimes M_3))~,\\
_{II} E_2^{p,q} \coloneqq \Hi{p}(\ZZ,\Hi{q}(\ZZ,M_1\otimes M_2)\otimes M_3)~.
\end{split}
\end{equation}
By Theorem \ref{thm:van-ff}, the entries, $E^{p,q}_2$ vanish if either $p<0$ or $q<0$, for both spectral sequences. Thus, we have $E_2^{00}=E_\infty^{00}$, which gives the isomorphism
$$
H^0_{tot}(C_{tot},d_{tot}) \cong \Hi{0}(\ZZ,M_1\otimes\Hi{0}(\ZZ,M_2\otimes M_3))\cong\Hi{0}(\ZZ,\Hi{0}(\ZZ,M_1\otimes M_2)\otimes M_3)~,
$$
as desired.
\end{proof}
Since the algebras $\V_{G,s}$ are free over $\ZZ_{<0}$ (Proposition $10.2$ of~\cite{Arakawa:2018egx}), the above lemma applies and FF-gluing $*_u$ is associative. We hold off on analysing associativity of $\ast$ for the twisted algebras, since it is hard to interpret the twisted FF gluing between two mixed vertex algebras.

How about mixing the two gluing operations, $\ast$ and $\circ$? 
\begin{lem}~\label{lem:rearr_gauge_ff}
Suppose  $U\in\ZZ$-Mod, $V\in\KL$ and $\W\in\KL$. Additionally, suppose $U$ is free over $\ZZ_{(<0)}$ and $W$ is semijective in $\KL$. Then we have the isomorphism
$$
U\ast(V\circ W) \cong (U\ast V)\circ W~.
$$
\end{lem}
\begin{proof}
Consider the bicomplex
$$
C^{\bullet\bullet} = U\otimes V\otimes W \Li{\bullet} (\zf(\gf))\otimes \Li{\bullet} (\gf)~,
$$
with differentials $d_\gf$ acting on $V\otimes W\otimes \otimes \Li{\bullet}(\gf)$ and $d_\zf$ acting on $U\otimes V \otimes \Li{\bullet}(\zf(\gf))$. The differentials anticommute and so we can form the total complex $C^p_{tot} = \bigoplus_{m+n=p} C^{p,q}$ with differential $d_{tot} = d_{\gf}+(-1)^q d_\zf$. There are two spectral sequences converging to the total cohomology:
\begin{equation}
	\begin{split}
	_I E_{2}^{p,q} = \Hi{p}(\ZZ, U \otimes \Hi{q}(\hat{\gf}_{-\kappa_g},\gf, V\otimes W))~,\\
	_{II} E_2^{p,q} = \Hi{p}(\hat{\gf}_{-\kappa_g},\gf,\Hi{q}(\ZZ,U \otimes V)\otimes W)~.
	\end{split}
\end{equation}
The cohmology $\Hi{p}(\ZZ,U\otimes - )$ vanishes for $p<0$ and the cohomology $\Hi{p}(\hat{\gf}_{-\kappa_g},\gf, - \otimes W)$ is concentrated in degree zero. Thus both spectral sequences will collapse at the second page and we have 
\begin{equation}
	_I E_2^{0,0} \cong\ _{II} E_2^{0,0} \cong H^0_{tot}(C_{tot},d_{tot})~,
\end{equation}
as desired
\end{proof}	

%For the special case of removing and adding punctures we have a powerful series of rearrangement lemmas regarding commutativity:

%\begin{lem}\label{lem:rearr_dsds}
%Let $V$ be a vertex algebra object in $\KL$ such that $H^0_{DS}(V)$ is also a vertex algebra object in $\KL$, where the reduction is taken with respect to any of the punctures. Let us label the punctures by $1,\dots,s$, then we have the following isomorphism
%$$
%H^0_{DS}(m,H^0_{DS}(n,V))\cong H^0_{DS}(n,H^0_{DS}(m,V))~,\quad \forall m,n\in\{1,\dots,s\}~,
%$$
%where $H^0_{DS}(i,-)$ is DS reduction with respect to the $i$th puncture.
%\end{lem}
%\begin{proof}
%This follows from Lemma \ref{lem:rearr_gauge} by using the isomorphism $H^0_{DS}(m,V) = \Hi{0}(\hat{\gf}_{-\kappa_g},\gf,\W\otimes V)$, where the action of $\hat{\gf}_{-\kappa_g}$ is via $\iota_m$.
%\end{proof}

%\begin{lem}\label{lem:rearr_capcap}
%Suppose $V$ is a vertex algebra with $s$ maximal punctures. We can label these punctures by $1,\dots,s$. The operation $\W_m\ast V$ introduces new punctures, the subscript $m$ corresponds to the label of this new puncture. Then, we claim that 
%$$
%\W_m\ast(\W_n \ast V) \cong \W_n \ast(\W_n \ast V) 
%$$
%\end{lem}
%\begin{proof}
%This is a corollary of Lemma \ref{lem:rearr_ff}, where $\W_m$ and $\W_n$ play the role of $M_1$ and $M_3$ in the proof of that lem.
%\end{proof}
%Thus, we justify our labelling of the vertex algebras $\V_{G,s}$ by the number of punctures. The order in which we add punctures is irrelevant and so is the order in which we remove them. Mixing the two operations, we have:

%\begin{lem}\label{lem:rearr_dscap}
%The functors $\Hi{0}(\ZZ,\W\otimes-):\ZZ\rightarrow\KL$ and $H^0_{DS}(-):\KL\rightarrow\ZZ$ commute in the sense that, if $M\in\KL$,
%$$ H^0_{DS}(\Hi{0}(\ZZ,\W\otimes M)) \cong \Hi{0}(\ZZ,\W\otimes H^0_{DS}(M))~.$$
%\end{lem}
%\begin{proof}
%For the special case where $M\cong H^0_{DS}(M^\prime)$ for some $M^\prime\in\KL$, this is just Theorem $9.11$ of~\cite{Arakawa:2018egx} and both sides are just the identity functor on $M$. 

%In general, we consider the bicomplex
	%$$
	%C^{\bullet\bullet} = \W\otimes M \otimes \W \otimes \Li{\bullet}(\mathfrak{z}(\gf))\otimes \Li{\bullet}(\mathfrak{\gf})~,
%$$
%where we have used the isomorphism
%$$
	%H^\bullet_{DS}(M) = \Hi{\bullet}(\hat{\gf}_{-\kappa_g},\gf,\W\otimes M)~,
%$$
%to rewrite the DS reduction as a gauging operation.  The differentials are $d_\ZZ$ and $d_\gf$ acting on $\W\otimes M\otimes\Li{\bullet}(\mathfrak{z}(\gf))$ and on $M \otimes \W\otimes\Li{\bullet}(\gf)$ respectively. The two differentials satisfy $d_\ZZ d_\gf=d_\ZZ d_\gf=0$ and so we can form the total complex $C^{\bullet}_{tot}$ as usual. There are two spectral sequences converging to the total cohomology $H^\bullet_{tot}(C_{tot},d_{tot})$, whose second pages are given by 
%\begin{equation}\nonumber
%\begin{split}
%_I E^{p,q}_2 = \Hi{p}(\ZZ,\W\otimes H^q_{DS}(M))~,\\
%_II E^{p,q}_2 = H^{p}_{DS}(\Hi{q}(\ZZ,\W\otimes M))~.
%\end{split}
%\end{equation}
%The cohomology $H^{\bullet}_{DS}(M)$ is concentrated in degree zero since $M\in\KL$ and $H^0_{DS}(-):\KL\rightarrow \ZZ$-Mod is exact. Thus, the spectral sequence collapses on the second page giving the isomorphism
%$$
	%H^p_{tot}(C_{tot},d_{tot}) \cong H^0_{DS}(\Hi{p}(\ZZ,\W\otimes M))\cong \Hi{p}(\ZZ,\W\otimes H^0_{DS}(M))~.
%$$
%Setting $p=0$ gives us the desired isomorphism.
%\end{proof}
%The proof of this lemma, actually applies to all the higher derived functors, $\Hi{p}(\ZZ,\W\otimes-)$ for $p>0$, i.e.\ 
%\begin{equation}
	%H^0_{DS}(\Hi{p}(\ZZ,\W\otimes M)) \cong \Hi{p}(\ZZ,\W\otimes H^0_{DS}(M))~,\quad \forall p\in\IN~.
%\end{equation}
%However, the full significance of this statement is not obvious to us.

We must also consider rearrangements of twisted and untwisted gluings. The results here are limited;the spectral sequence arguments will often fail in the twisted setting, since the mixed vertex algebras are not expected to be semijective in $\KL_u$. Yet we are able to show some aspects of the twisted algebras are as we expect. To start with, we have a lemma regarding the interchange of twisted and untwisted gauging.
\begin{lem}\label{lem:gauge_ut}
Suppose $V_1$ is in $\KL_u$, $V_2$ is in $\KL_u$ and $\KL_t$, and $V_3$ is in $\KL_t$. Furthermore, suppose that $V_3$ is semijective, of Theorem~\ref{thm:gauge-van}, for $\gf_t$. Then, we have the isomorphism
$$
V_1\circ_u(V_2\circ_t V_3) \cong (V_1\circ_uV_2)\circ_tV_3~.
$$
\end{lem}
\begin{proof}
As usual, the proof is via spectral sequences, with the additional difficulty of cohomology not being concentrated in degree zero. We define the bicomplex
$$
C^{p,q} = V_1\otimes V_2\otimes V_3 \otimes \Li{p}(\hat{\gf}_u)\otimes \Li{q}(\hat{\gf}_t)~,
$$
with the differential $d_u$ and $d_t$ acting on $V_1\otimes V_2\otimes\Li{\bullet}(\hat{\gf}_u)$ and $V_2\otimes V_2\otimes \Li{\bullet}(\hat{\gf}_t)$ respectively. The differentials anticommute and so we can form the total complex $C_{tot}^m = \bigoplus_{p+q=m}C^{p,q}$ with the differential $d_{tot}= d_u +(-1)^p d_t$. There are two spectral sequences converging to the total cohomology, given by
\begin{equation}\nonumber
\begin{split}
_I E_2^{p,q} = \Hi{p}(\hat{\gf}_{u,-\kappa_g},\gf_u,V_1\otimes\Hi{p}(\hat{\gf}_{t,-\kappa_g},\gf_t,V_2\otimes V_3))~,\\
_{II} E^{p,q}_2 = \Hi{p}(\hat{\gf}_{t,-\kappa_g},\gf_t,\Hi{q}(\hat{\gf}_{u,-\kappa_g},\gf_u,V_1\otimes V_2)\otimes V_3)~. 
\end{split}
\end{equation}
Since $V_3$ satisfies the conditions of Theorem~\ref{thm:gauge-van}, the spectral sequences will collapse on the second page and $_1 E^{p,q}_2=0$ for $q<0$ and $_{II} E^{p,q}_2 =0$ for $p<0$. Thus we have the isomorphism 
$$
H^m_{tot} =\, _I E^{m,0}_2 =\, _{II} E^{0,m}_2
$$
\end{proof}
Additionally, we can also show that the twisted gauging and untwisted FF-gluing play together nicely.
\begin{lem}\label{lem:ut-cap-gauge}
Let $M$ be an object of $\ZZ_u$-Mod such that it is free over $\ZZ_{u,<0}$ and let $W$ be semijective in $\KL_t$. Suppose, $V$ is a vertex algebra object in $\KL_t$, then we have the isomorphism.
$$
M\ast_u(V\circ_t W)\cong (M\ast_u V)\circ_t W~.
$$
\end{lem}
\begin{proof}
Let $C^{p,q}$ be the bicomplex
$$
C^{p,q} = M\otimes V\otimes W \otimes \Li{p}(\mathfrak{z}(\gf_u))\otimes \Li{q}(\hat{\gf}_t)~,
$$
with the differentials $d_\mathfrak{z}$ acting on $M\otimes V\otimes \Li{\bullet}(\mathfrak{z}(\gf_u))$ and $d_{\gf}$ acting on $V\otimes W \Li{\bullet}(\hat{\gf_t})$. The differentials $d_\mathfrak{z}$ and $d_\gf$ anticommute and so we can form the total complex $C^m_{tot} = \bigoplus_{p+q=m}C^{p,q}$ with the total differential $d_{tot}=d_\mathfrak{z}+(-1)^p d_\gf$. There are two spectral sequences converging to the total cohomology, given by
\begin{equation}\nonumber
\begin{split}
	_I E^{p,q}_2 = \Hi{p}(\ZZ_u,M\otimes\Hi{q}(\hat{\gf}_{t,-\kappa_g},\gf_t,V\otimes W))~,\\
	_{II} E^{p,q}_2 = \Hi{p}(\hat{\gf}_{t,-\kappa_g},\gf_t,\Hi{q}(\ZZ_u,M\otimes V)\otimes W)~.
	\end{split}
\end{equation}
The cohomology $\Hi{q}(\hat{\gf}_{t,-\kappa_g},\gf_t,-\otimes W)$ is concentrated in degree zero, and so both spectral sequence will collapse in the second page. Thus, we have the isomorphism
$$H^0_{tot}(C_{tot},d_{tot}) \cong _I E^{0,0}_2 \cong _{II} E^{0,0}_2~.$$
\end{proof}

%\subsection{The character of twisted trinions}
%\label{ssec:fixtures/character}

%A consistency check we should make is whether the characters of these mixed vertex algebras agree with the superconformal indices of physics. It will turn out that Proposition~\ref{prop:cyl_kl0} is sufficient to compute the characters of the mixed vertex algebras.

%As a vertex algebra object in $\KL_u$, the mixed trinion admits a decomposition
%\begin{equation}
%\V_{1,1} = \bigoplus_{\lambda' \in P^+_u} \V_{1,1}^{[\lambda']}~,
%\end{equation}
%into modules of $\hat{\gf}_{u,\kappa_c}$. The twisted cylinder on the other hand admits a decomposition
%\begin{equation}
	%\D_t \cong \bigoplus_{\lambda\in P^+_t} \IV^t_\lambda\otimes\IV^t_{\lambda^*}~,
%\end{equation}
%as graded vector spaces.

%Proposition $8.4$ of Arakawa, relates the character of $\V_{1,1}^{[\lambda']}$ to $H^0_{DS}(\V_{1,1}^{[\lambda']})$. From Proposition~\ref{prop:cyl_kl0} and our arguments for Theorem~\ref{thm:closed_immersion}, we know that
%\begin{equation}
	%H^0_{DS} (\V_{1,1}^{[\lambda']}) \cong 0~,
%\end{equation}
%unless $\lambda'$ is in the image of $\iota:P_t^+\hookrightarrow P_u^+$. In the cases where $\lambda'=\iota(\lambda)$, we have
%\begin{equation}
	%H^0_{DS}(\V_{1,1}^{[\lambda]}) \cong \IV^t_{\lambda}\otimes\IV^t_{\lambda^*}
%\end{equation}
%as graded vector spaces. From Proposition $8.4$ of Arakawa, we have that
%\begin{equation}
	%\mathrm{ch}\,{\V_{1,1}^{[\lambda]}} = q^{(\lambda|\rho^\vee)}\mathrm{ch} \, \mathbb{L}^u_\lambda \mathrm{ch}\, \IV^t_{\lambda}\otimes \IV^t_{\lambda^*}~,
%\end{equation}
%where $\mathbb{L}^u_\lambda$ is the simple quotient of the Weyl module $\IV^u_{\lambda}$. The characters of these objects are well known and we find that
%\begin{equation}
	%\mathrm{ch}\,{\V_{1,1}^{[\lambda]}} = \frac{\KK_u(\mathbf{a})\chi_u^\lambda(\mathbf{a})\KK_t(\mathbf{b}_1)\chi_t^\lambda(\mathbf{b}_1) \KK_t(\mathbf{b}_2)\chi_t^\lambda(\mathbf{b}_2)}{\KK_u(\times)\chi^\lambda_t(\times) }~.
%\end{equation}
%Thus, the character of $\V_{1,1}$ is given by
%\begin{equation}
	%\mathrm{ch}_{\V_{1,1}}(\mathbf{a},\mathbf{b}_1,\mathbf{b}_2) = \sum_{\lambda\in P^+_t} \frac{\mathcal{K}_u(\mathbf{a})\mathcal{K}_t(\mathbf{b}_1)\mathcal{K}_t(\mathbf{b}_2)\chi^{\lambda}_u(\mathbf{a})\chi^{\lambda}_t(\mathbf{b}_1)\chi^{\lambda}_t(\mathbf{b}_2)}{\mathcal{K}_u(\times)\chi_u^{\lambda}(\times)}~,
%\end{equation}
%Note that the sum is restricted to the weights in the image $P_t^+\hookrightarrow P_u^+$ as in~\cite{Lemos:2012ph}.

%This agrees with the expression for the superconformal index of~\cite{Lemos:2012ph}. Since all other surfaces are obtained by gauging copies of $\V_{1,1}$, the characters of $\V_{m,n}$ should agree with the superconformal indices of the corresponding theories.


%All this relies on the assumption that the vertex algebra $\V_{1,1}$ is conformal. We believe that this is a fairly reasonable assumption to make, indeed both $\D_t$ and $\W_u$ are conformal vertex algebras. Since $H^0_{DS}(u,\V_{1,1})\cong \D_t$ by Proposition~\ref{prop:cyl_kl0}, we can construct a candidate for the conformal vector of $\V_{1,1}$. The conformal vector of a DS reduced vertex algebra can be related to the conformal vector of the unreduced theory very explicitly --- see~\cite{Beem:2014kka} for instance. Inverting this relation, we would expect
%\begin{equation}
	%T_{\V_{1,1}} = T_{\D_t} + \partial \Lambda(h) +\partial b_\alpha c^\alpha - (1+\lambda_\alpha)\partial (b_\alpha c^\alpha) + \QQ_{DS}\text{-exact terms}~,
%\end{equation}
%where $\Lambda(h)$ is the image of the Cartan element of $\mathfrak{sl}_2$ in the  $V^\kappa_{c}(\gf_u)$ subalgebra of $\V_{1,1}$, $(b_\alpha,c^\alpha)$ are the BRST ghosts involved in the DS reduction, and $\lambda_\alpha$ is the weight of the generator $t_\alpha\in\gf_u$ under $\Lambda(h)$. There is of course an ambiguity in this expression, it is only defined up to $\QQ_{DS}$-exact terms. The central charge on the other hand can be exactly computed by inverting a similar relation. We have
%\begin{equation}
	%c_{\V_{u=1,t=3}} = c_{\D_t} - \mathrm{rk}\,\gf_t + \frac{1}{2}\dim\,\gf_{t,1/2} -24\rho_{\gf_t}\cdot\rho_{\gf_t^\vee}-\dim \gf_t~,
%\end{equation}
%where $\gf_{t,1/2}$ is the component with eigenvalue $1/2$ under the image $\Lambda(h)$ and $\rho$ is the Weyl vector. % insert FFR as justification?

%Given two vertex algebras $V_1$ and $V_2$ with conformal vectors, $T_1$ and $T_2$, we can construct the conformal vector for the gauged vector algebra $V_1\circ V_2$ as
%\begin{equation}
	%T = T_1 + T_2 + T_{gh}
%\end{equation}
%where $T_{gh}$ is the conformal vector for the $(b,c)$ ghost vertex algebra. With this choice of conformal vector, the central charge of $\V_{m,n}$ agrees with the expression in~\cite{Chacaltana:2012zy}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Mixed vertex algebras at genus zero}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We begin with proposing a construction of the vertex algebras associated to $\CC_{0,m,1}$ before considering the more general case. Much like the untwisted case, one could define $\V_{m,1}$ recursively by gluing untwisted caps. We shall elect, instead, to perform a simultaneous gluing --- analogous to the construction of $\V_{G,s}$.
We define the vertex algebras $\V_{m,1}$ by 
\begin{equation}
\begin{split}
\V_{0,1} &\coloneqq \D_t~,\\
	\V_{m,1} &\coloneqq H^0(C_{m,1},Q^m)~,
\end{split}
\end{equation}
where $C_{m,1}$ is the chain complex
\begin{equation}
	C^{\bullet}_{m,1} =  \W_u^m \otimes \D_t \otimes\bigg( \Li{\bullet}(\zf(\gf_u))\bigg)^{m} ~,
\end{equation}
with differential
\begin{equation}
	\begin{split}
	Q^{m}(z) &= \sum_{i=1}^{m}Q^{i,i+1}~,\\
	Q^{i,i+1}(z) &= \sum_{j=1}^{\mathrm{rk}\,\gf_u} : (\rho_i(P_j) -\rho_{i+1}(\tau(P_j)))\rho_{gh_{i}}(c^j):(z)~,
	\end{split}	
\end{equation}
where $\rho_i$, for $i\le m$ denote the action of $\zf(\gf_u)$ on the $i$th factor of $\W_u$ and $\rho_{m+1}$ denotes the action of $\zf(\gf_u)$ on $\D_t$ along the projection $\ZZ_u\twoheadrightarrow \ZZ_t$. One should think of this as the \textit{simultaneous} gluing of $m$ caps to the twisted cylinder. The similarity to Arakawa's construction is manifest and, indeed, the vertex algebras $\V_{m,1}$ shall enjoy many of the properties of their untwisted counterparts.
By construction, the vertex algebras $\V_{m,1}$ have no fermions, since we restrict to the zeroth cohomology --- agreeing with our discussion on residual gauge symmetries.
We shall later reinforce this by showing that the cohomology of $\V_{m,1}\circ_t\V_{n,1}$ is concentrated in degree zero.


 A generalisation to $\V_{m,n}$ of our previous construction would be to take the zeroth cohomology of 
\begin{equation}
	C^{\bullet}_{m,n} = \W^{m}_u\otimes \V_{G_t,2n} \otimes \bigg( \Li{\bullet}(\zf(\gf_u))\bigg)^{m}~.
\end{equation}
However, this cannot be the case. We have argued that there is residual gauge symmetry in the theories associated to $\CC_{0,m,n}$ for $n>1$ and thus one should see fermions in the corresponding vertex algebra. The vertex algebras, $\W_u$ and $\V_{G_t,2n}$, have no fermions, and since we truncate to zeroth cohomology, neither can the proposed construction. One should also expect to see a $\IZ_2$ ghost-anti-ghost symmetry in the cohomology which swaps positive and negative cohomology. The untwisted caps $\W_u$ are projective over $\ZZ_{u,(<0)}$ and the cohomology vanishes in negative degree. Therefore, even if we do not truncate to zero cohomology the resulting vertex algebra does not have the required $\IZ_2$ symmetry.

We have shown, in our discussion of the rearrangement lemmas that one must be wary in rearranging the order of gluings when both untwisted and twisted gluings are present. This immediately presents a hurdle in defining the vertex algebras associated to $\CC_{0,m,n}$. In one duality frame, these can be obtained as $\CC_{0,m+1,n-1}\circ_u\CC_{0,1,1}$ whereas in another they can decompose as $\CC_{0,m-1,n}\circ_t \CC_{0,1,1}$. It is not, \textit{a priori}, obvious that the two decompositions will agree --- both the type of gluing and the ingredients are different.

These considerations, force us to define the vertex algebras, $\V_{m,n}$, by going to a specific duality frame. Specifically, consider driving the complex structures of $\CC_{0,m,n}$ to the point where it decomposes as $\CC_{0,m+1,n-1}$ and $\CC_{0,1,1}$ connected by an untwisted cylinder. This is the intuition behind our recursive definition:
\begin{equation}
	\V_{m,n}\coloneqq \V_{1,1}\circ_u\V_{m+1,n-1}~.
\end{equation}
Unlike the $\V_{m,1}$, we have had to choose, non-canonically, some duality frame to define the vertex algebras for surfaces with more than one pair of twisted punctures. As defined, it is not clear whether the $\V_{m,n}$ are independent of such a choice. In the following sections, we shall work to establish how our definitions fit in with the duality web of Class $\SS$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\label{ssec:gluing_mixed}Properties of the genus zero mixed vertex algebras}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

First, we wish to check our definition of the mixed vertex algebras agrees with the recursive definition, $\V_{m,1}\overset{?}{\cong} \W_u\ast_u \V_{m-1,1}$ and so we present an extension of Lemma $10.1$ of Arakawa to the twisted case. 

\begin{lem}\label{lem:mix_ff_cap}
For $m\ge 1$, we have that 
\begin{enumerate}[(i)]
	\item $H^{n}(C_{m,1},Q^{m-1}_{(0)}) \cong 0\text{ for } n<0~,$
	\item $\W_u\ast_u \V_{m-1,1} \cong \V_{m,1}~.$
\end{enumerate}
\end{lem}
\begin{proof}
This proof is largely adapted from the proof of Lemma $10.1$ in~\cite{Arakawa:2018egx}.
We proceed by induction on $m$. For the base case, $m=1$, $(i)$ is true, since $\W_u$ is projective over $\ZZ_{u,(<0)}$. The second statement is true by definition, since $\V_{1,1}\coloneqq \W_u\ast_u\D_t$. Next, suppose $m>1$ and consider the bicomplex
$$
C^{\bullet\bullet} = \W_u\otimes C_{m-1,1}^\bullet \otimes \Li{\bullet}(\zf(\gf_u))~,
$$
with differentials $Q^{m-1}_{(0)}$ acting on $C_{m-1,1}$ and $d$ acting on $\W_u\otimes C_{m-1,1}\otimes \Li{\bullet}(\zf(\gf_u))$. The two differentials anticommute and the total complex is just $C_{m,1}$ with differential $Q^{m}_{(0)}$. 
There is a spectral sequence, with second page 
$$
E_{2}^{p,q} = \Hi{p}(\ZZ_u, \W_u\otimes H^{q}(C_{m-1,1},Q^{m-1}_{(0)}))~,
$$
which converges to the total cohomology. By the inductive assumption, $H^{q}(C_{m,1},Q^{m-1}_{(0)})$ vanishes for $q<0$ and $\W_u\ast_u-$ is left exact. Therefore, $E_{2}^{p,q}=0$ for $p<0,q<0$ and so $H^{n}(C_{m,1},Q^m_{(0)})$ vanishes for $n<0$. Moreover, the entry $E_{2}^{0,0}$ is stable and we have 
\begin{equation}
	E_2^{0,0} = \W_u\ast_u \V_{m-1,1} \cong H^{0}(C_{m,1},Q^{m}_{(0)})\cong \V_{m,1}~,
\end{equation}
as desired.
\end{proof}

Next, we examine the case of untwisted DS reduction.
\begin{lem}\label{lem:mix_kl0}
The mixed vertex algebras $\V_{m,n}$ are objects in $\KL_{u,0}$. In particular, for $m\ge 0$ and $n\ge 1$
$$
H^0_{DS}(u, \V_{m+1,n}) \cong \V_{m,n}~.
$$ 
\end{lem}
\begin{proof}
We proceed by double induction on $m$ and $n$, first examining the base case of $n=1$ and arbitrary $m$.
Note that for $m=0$, $H^0_{DS}(u,\V_{1,1})=\D_t$ from Theorem~\ref{thm:cyl_kl0}. Next, suppose $m>0$; for any object in $\KL_u$, $H^0_{DS}(u,-)$ and $\W_u\circ_u-$ are isomorphic. Therefore,
$$
H^0_{DS} (u,\V_{m+1,1}) \cong \W_u\circ_u \V_{m+1,1}\cong \W_u \circ_u(\W_u\ast_u \V_{m,1})~,
$$
where we have used Lemma~\ref{lem:mix_ff_cap}.
Consider the bicomplex
$$
C^{\bullet \bullet} =\W_u\otimes \V_{m,1}\otimes \W_u \otimes \Li{\bullet}(\zf(\gf_u))\otimes \Li{\bullet}(\hat{\gf}_{u,-\kappa_g})~,
$$
with differential $d_\gf$ acting on $\W_u\otimes \V_{m,1} \otimes \Li{\bullet}(\hat{\gf}_{u,-\kappa_g})$ and $d_\zf$ acting on $\V_{m,1}\otimes \W_u \otimes \Li{\bullet}(\zf(\gf_u))$. The two differentials anticommute and so we form the total complex $C^n_{tot}=\bigoplus_{p+q=n} C^{pq}$, with total differential $d_{tot} = d_{\gf} + (-1)^q d_\zf$. There are two spectral sequences converging to the total cohomology, given by
\begin{equation}\nonumber
	\begin{split}
	_I E^{pq}_2 &= \Hi{p}(\ZZ_u,\W_u\otimes \Hi{q}(\hat{\gf}_{u,-\kappa_g},\gf_u,  \V_{m,1}\otimes \W_u))~,\\
	_{II} E^{pq}_2 &= \Hi{p}(\hat{\gf}_{u,-\kappa_g},\gf_u ,\Hi{q}(\ZZ_u,\W_u\otimes \V_{m,1})\otimes W_u)~.
	\end{split}
\end{equation}
The cohomology, $\Hi{\bullet}(\hat{\gf}_{u,-\kappa_g},\gf_u,-\otimes \W_u)$ is concentrated in degree zero, and $\Hi{i}(\ZZ_u \W_u\otimes -)$ vanishes for $i<0$. Therefore, both spectral sequences collapse at the second page and we have 
\begin{equation}\nonumber
	\W_u\ast_u(\W_u\circ_u \V_{m,1})=\ _I E^{00}_2\cong\ _{II} E^{00}_2 =\W_u\circ_u(\W_u\ast_u \V_{m,1})~.
\end{equation}
Therefore, 
$$
H^0_{DS}(u,\V_{m+1,1}) \cong \W_u\ast_u (\W_u\circ_u\V_{m,1})\cong \W_u \ast_u (H^0_{DS}(u,\V_{m,1})~,
$$
but $\W_u\ast_u(H^0_{DS}(u,\V_{m,1}))\cong \V_{m,1}$ by Theorem 9.11 of~\cite{Arakawa:2018egx}.

Now suppose $n>1$. Then, we have that 
$$
H^0_{DS}(u,\V_{m+1,n}) \cong \W_u\circ_u(\V_{1,1}\circ_u \V_{m+2,n-1})~.
$$
Since, $\W_u$ is semijective in $\KL_u$, Lemma~\ref{lem:rearr_gauge} applies and so we have that 
\begin{equation}\nonumber
\begin{split}
	H^0_{DS}(u,\V_{m+1,n}) &\cong \V_{1,1}\circ_u(\W_u\circ_u\V_{m+2,n-1})~,\\
	&\cong \V_{1,1} \circ_u (H^0_{DS}(u,\V_{m+2,n-1}))~,\\
	&\cong \V_{1,1}\circ_u \V_{m+1,n-1}~,
\end{split}
\end{equation}
where we have used the inductive assumption. Of course, $\V_{1,1}\circ_u \V_{m+1,n-1}$ is $\V_{m,n}$ by definition and so we are done.
\end{proof}
Our uniqueness result for $\V_{1,1}$ can now be extended to all of the genus zero vertex algebras $\V_{m,n}$. To reiterate, $\V_{m,n}$ is the unique vertex algebra object in $\KL_u^{\otimes m}$ such that $H^0_{DS}(u, \V_{m-1,n})$.

Using Lemma~\ref{lem:mix_kl0}, we can present our version of Proposition $10.10$ of~\cite{Arakawa:2018egx}.
\begin{prop}\label{prop:mixed_free_cofree}
The vertex algebras $\V_{m,1}$ have an ascending filtration whose successive quotients are
$$
\IV^u_{\lambda,m}\otimes_{\zf^u_{\lambda}}(\IV^t_{\lambda}\otimes_{\zf^t_\lambda}\IV^t_{\lambda*})~,
$$
for some $\lambda\in P_t^+$ and $\iota(\lambda)\in P_u^+$.
Additionally, the vertex algebras $\V_{m,1}$ have a descending filtration whose successive quotients are 
$$
D\big(
\IV^u_{\lambda,m}\otimes_{\zf^u_{\lambda}}(\IV^t_{\lambda}\otimes_{\zf^t_\lambda}\IV^t_{\lambda*})\big)~.
$$
Therefore, the vertex algebras $\V_{m,1}$
are semijective in $\KL_t$ and so 
$$
\V_{m,1}\circ_t V \cong \Hi{0}(\hat{\gf}_{t,\kappa_g},\gf,\V_{m,1}\otimes V)~.
$$
\end{prop}
\begin{proof}
First, note that the objects $\IV_{\lambda,m}\otimes_{\zf^u_{\lambda}}(\IV^t_{\lambda}\otimes_{\zf^t_\lambda}\IV^t_{\lambda*})\big)$ are in $\KL_u,0$, by the same argument as Proposition~\ref{prop:kl_u}. 
We proceed via induction, noting that for the base case $m=1$ the statement is true by way of Proposition~\ref{prop:trin_free_cofree}. 

Suppose the statement is true for some $m>1$,~\ie\ $\V_{m,1}$ has a filtration 
$$
0=N_0\subset N_1\subset \dots \subset N=\bigcup_i N_i
$$
with successive quotients $N_i/N_{i-1}\cong \IV_{\lambda,m}\otimes_{\zf^u_\lambda}((\IV^t_{\lambda}\otimes_{\zf^t_\lambda}\IV^t_{\lambda*})$ for some $\lambda\in P_t^+$ and $\iota(\lambda)\in P_u^+$.
we have
$$
	\V_{m+1,1} \cong \W_u\ast_u\V_{m,1}~,
$$
by Lemma~\ref{lem:mix_ff_cap}. By Proposition $9.14$ of~\cite{Arakawa:2018egx}, $\V_{m+1,1}$ has an ascending filtration 
$$
0=M_0\subset M_1\subset\dots\subset M = \bigcup_i M_i ~,
$$
with successive quotients $M_i/M_{i-1}\cong \W_u\ast_u N_i/N_{i-1}$. Since $N_i/N_{i-1}$ are objects in $\KL_{u,0}$, we have that 
$$
M_i/M_{i-1} \cong \IV_{\lambda,m+1}\otimes_{\zf^u_\lambda}((\IV^t_{\lambda}\otimes_{\zf^t_\lambda}\IV^t_{\lambda*})~,
$$
for some $\lambda\in P_t^+$ and $\iota(\lambda)\in P_u^+$.
\end{proof}
One could hope to strengthen this to the statement that all $\V_{m,n}$ are semijective in $\KL_t$ but this is beyond us for the moment. With our current argument, we would have to independently establish that the vertex algebras $\V_{0,n}$ are semijective in $\KL_{u,0}$. Given that our definition of $\V_{0,n}$ involves an unbounded cohomology, it seems difficult to verify such a property.

From a similar argument as with $\V_{1,1}$, the mixed vertex algebra, $\V_{m,1}$ cannot be semijective in $\KL_u$ and so the derived functor $\V_{1,1}\circ_u-$, which increases the number of pairs of twisted punctures by one, is not concentrated in degree zero. By construction, the $\V_{m,n}$ cannot be concentrated in cohomological degree zero for $n>1$. This is, in one sense, a good thing --- going back to our discussion on residual gauge symmetry, these vertex algebras should have fermions present. On the other hand, this is a rather large roadblock to our spectral sequence powered proofs of associativity. We will only be able to provide partial results for how $\V_{m,n}$ fit in the duality web. 

Similar to the mixed trinion, we can derive the characters and central charges of the mixed vertex algebras.
\begin{prop}\label{prop:mixed_char}
The character of the vertex algebra $\V_{m,1}$ is given by
$$
\Tr_{\V_{m,1}}\bigg(q^{L_0}\prod_{i=1}^{m} \mathbf{a}_i \,\,\mathbf{b}_1\mathbf{b}_2\bigg) =  \sum_{\lambda\in P_t^+} \frac{\prod_{i=1}^m \KK_u(\mathbf{a}_i)\chi^\lambda_u(\mathbf{a}_i)  \KK_t(\mathbf{b}_1)\chi^\lambda_t(\mathbf{b}_1) \KK_t(\mathbf{b}_2)\chi^\lambda_t(\mathbf{b}_2) }{\big( \KK_u(\times)\chi^\lambda_u(\times) \big)^{m}}~.
$$
and so the vertex algebra, $\V_{m,1}$ is conical for all $m\in \IN$.
\end{prop}
\begin{proof}
For $m=1$ this is just Proposition~\ref{prop:mixed_trin_char}, so we take $m>1$. We have that $H^0_{DS}(u,\V_{m,1})\cong \V_{m-1,1}$. As graded vector spaces, we have the decomposition
$$
\V_{m-1,1} \cong \sum_{\lambda\in P_t^+} \IV^u_{\lambda,m-1} \otimes_{\zf_\lambda^u}(\IV^t_{\lambda}\otimes_{\zf_\lambda^t}\IV^t_{\lambda*})~.
$$
Applying Proposition~8.4 of~\cite{Arakawa:2018egx} gives us the desired result. The fact that $\V_{m,1}$ are conical follows from the same argument as Proposition~\ref{prop:mixed_trin_char}.
\end{proof}

The vertex algebra $\V_{m,n}$ is constructed by repeatedly gauging $\V_{m+n-1,1}$ with copies of $\V_{1,1}$. We know how the character behaves under gauging, and so this result can be extended to
\begin{equation}\label{eq:mixed_char}
	\Tr_{\V_{m,n}}\bigg(q^{L_0}\prod_{i=1}^{m} \mathbf{a}_i \,\prod_{j=1}^{2n}\mathbf{b}_j\bigg)=\frac{\prod_{i=1}^m \KK_u(\mathbf{a}_i)\chi^\lambda_u(\mathbf{a}_i) \prod_{j=1}^{2n} \KK_t(\mathbf{b}_j)\chi^\lambda_t(\mathbf{b}_j)} {\big( \KK_u(\times)\chi^\lambda_u(\times) \big)^{m+2n-2}}~,
\end{equation}
which agrees with the expression in~\cite{Lemos:2012ph}.

\begin{prop}
The vertex algebras $\V_{m,1}$ are conformal with central charge 
$$
c_{\V_{m,1}} = m\,\dim \gf_u + 2\dim \gf_t -24m\,\rho_u\cdot\rho_u^\vee -m\, \rk\,\gf_u~.
$$
\end{prop}
\begin{proof}
From Proposition~\ref{prop:mixed_trin_conf}, we know that $\V_{m,1}$ is conformal with central charge $c_{\V_{1,1}} = 2\dim\, \gf_t + \dim\,\gf_u -\rk\,\gf_u -24 \rho_u\cdot\rho_u^\vee$ and so the statement is true of $m=1$. 

We shall first show that $\V_{m,1}$ has a conformal vector, then show that it is the unique conformal vector whose grading agrees with the character and finally show that this results in the 
correct central charge.

Consider the vector $\omega_m\in C_{m,1}$, defined by 
$$
	\omega_m = \omega_{\D_t} + \sum_{i=1}^{m} \omega_{\W_i}+\sum_{i=1}^m \omega_{gh,i} ~,
$$
where $\omega_{\D_t}$ is the conformal vector of $\D_t$, $\omega_{\W_i}$ is the conformal vector of the $i$th factor of $\W_u$ and $\omega_{gh,i}$ is the conformal vector of the $i$th ghost system, $\Li{\bullet}(\zf(\gf_u))$. Clearly, $\omega_m$ defines a conformal vector on the complex, $C_{m,1}$. Like we did for $\V_{1,1}$ we shall argue that this descends to a conformal vector in cohomology.

For an element $P_i\in\zf(\gf_u)$, where we think of $\zf(\gf_u)$ as a subalgebra of one of the $\W_u$ factors, $\omega_m$ acts as 
$$
\omega_m(z) P_i(w) \sim \frac{\partial P_i}{z-w} +\frac{(d_i+1) P_i}{(z-w)^2}+\sum_{j=2}^{d_i+2}\frac{(-1)^j j!}{(z-w)^{j+1}} q_j^{(i)}(w)~,
$$
where $q_j^{(i)}$ is some homogeneous state in $\zf(\gf_u)$ with weight $d_i-j+2$. Let us denote by $\widetilde{P_i}$ the image of $P_i$ under the projection $\zf(\gf_u)\twoheadrightarrow \zf(\gf_t)$.
One then has
$$
\omega(z) \widetilde{P_i}(w) \sim \frac{\partial \widetilde{P_i}}{z-w} +\frac{(d_i+1) \widetilde{P_i}}{(z-w)^2}+\sum_{j=2}^{d_i+2}\frac{(-1)^j j!}{(z-w)^{j+1}} \widetilde{q_j}^{(i)}(w)~,
$$
where we think of $\widetilde{P_i}$ as a state in $\zf(\gf_t)\subset\D_t$. Let $Q^m$ be the differential of $C_{m,1}$; the action of $Q^m$ on the vector $\omega_m$ is
$$
Q^m_{(0)}(z) \omega(w) = \sum_{l=1}^{m}\sum_{i=1}^{\mathrm{rk}\,\gf_u}\sum_{j=2}^{d_i+1} \partial^j \big(\rho_l(q_j^{(i)}) -\rho_{l+1}(\tau(q^{(i)}))\big)c_i ~,
$$
where $\rho_i$, for $i\le m$ denote the action of the Feigin-Frenkel centre on the $i$th $\W_u$ factor and $\rho_{m+1}$ once again denotes the action of $\zf(\gf_u)$ on $\D_t$ along the projection to $\zf(\gf_t)$.

If the right hand side of the above equation equals $Q^m_{(0)}\chi$ for some state $\chi$, then $\widetilde{\omega}_m = \omega_m + \chi$ is $Q$-closed and defines a vector in $\V_{m,1}$.
For $l\neq m$ it is clear that $\rho_l(q_j^{(i)})-\rho_{l+1}(q_j^{(i)})$ is a coboundary, and we have addressed the $l=m$ case in the proof of Proposition~\ref{prop:mixed_trin_conf}. Therefore, such a $\chi$ exists and may be written as
$$
\chi = \sum_{l=1}^m\sum_{i=1}^{\mathrm{rk}\, \gf_u}\sum_{j=2}^{d_i+2} \partial^j (\rho_{l}\otimes \rho_{l+1}\otimes \rho_{gh,l})(z_{ij})
$$
for some $z_{ij} \in \zf(\gf_u)\otimes\zf(\gf_u)\otimes \Li{0}(\zf(\gf_u))$. Therefore, $\widetilde{\omega}_{m,(i)}=\omega_{m,(i)}$ for $i=0,1$, and so the OPEs agree up to the quadratic pole. 
Since $\V_{m,1}$ is conical by Proposition~\ref{prop:mixed_char}, Lemma $3.1.2$ of~\cite{Frenkel:2007} applies once more and we can conclude that $\widetilde{\omega}_m$ is a conformal vector in $\V_{m,1}$.

%says that all we need to check is that $\widetilde{\omega}_{(3)}\widetilde{\omega}= c/2\ket{0}$ for some $c\in\IC$.,~\ie\ the quartic pole in the Virasoro-Virasoro OPE is a multiple of the identity. 

%However, we know that $\V_{1,1}$ is conical from its character and so the only operator of dimension zero that can appear in the OPE is the identity. Thus, $\widetilde{\omega}$ is a conformal vector of $\V_{1,1}$.

Now we wish to show that $\widetilde{\omega}_m$ is the unique conformal vector whose $L_0$-grading agrees with $\omega_m$. The argument from Proposition~\ref{prop:mixed_trin_conf} using Lemma 4.1 of~\cite{Moriwaki_2020} still works, with minor alteration, since $\V_{m,1}$ are conical.

The DS reduction of $\widetilde{\omega}_m$ gives a conformal vector in $\V_{m-1,1}$ with central charge
$$
c_{\V_{m-1,1}} = c_{\V_{1,1}} +\rk\,\gf_u - \dim \gf_{u} +24 \rho_{u}\cdot\rho^\vee_{u}~,
$$
and which agrees with the grading by $\omega_{m-1}$. But, by the inductive assumption, such a conformal vector on $\V_{m-1,1}$ is unique.

Unwrapping the induction from the base case of $\V_{0,1}=\D_t$, we get that
$$
c_{\V_{m,1}} = m\,\dim \gf_u + 2\dim \gf_t -24m\,\rho_u\cdot\rho_u^\vee -m\, \rk\,\gf_u~.
$$
\end{proof}

To extend this to $\V_{m,n}$, we shall once more make use of the fact the $\V_{m,n}$ are constructed by repeated twisted gaugings of the $\V_{m,1}$ with copies of $\V_{1,1}$. It is well known that the conformal vector 
\begin{equation}
T = \widetilde{\omega}_{\V_{k,l}} + \widetilde{\omega}_{\V_{1,1}} +\omega_{gh} ~,
\end{equation}
where $\omega_{gh}$ is the conformal vector of the $b,c$ ghost system, descends to a conformal vector in the BRST cohomology with central charge  equal to the central charge of $T$. Therefore the vertex algebras $\V_{m,n}$ are conformal, with central charge
\begin{equation}
	c_{\V_{m,n}} = 2n\, \dim\,\gf_t + m\, \dim\,\gf_u - (m+2n-2)\rk\,\gf_u -24(m+2n-2)\,\rho_u\cdot\rho_u^\vee~.
\end{equation}

Having established a number of intrinsic properties of the genus zero, mixed vertex algebras, let us examine how they interact with each other under gluing. This will shed some light on how the $\V_{m,n}$ fit into the class $\SS$ duality web.

Given our rearrangement lemmas, we can show that the mixed vertex algebras of the previous section have the expected behaviour under $\circ_u$ and $\circ_t$. First, we establish the partial result

\begin{lem}\label{lem:gauge_mix_trin}
We have the isomorphism
$$
\V_{1,1}\circ_t \V_{m,n} \cong \V_{m+1,n}~.
$$
\end{lem}
\begin{proof}
First, let us treat the base case of $n=1$. We have that 
$$
	\V_{1,1}\circ_t \V_{m,1} \cong (\W_u \ast_u \D_t)\circ_t \V_{m,1}~,
$$
and so $\V_{1,1}\circ_t \V_{m,1} \cong \W_u\ast_u \V_{m,1} \cong \V_{m+1,1}$.
By Lemma~\ref{lem:ut-cap-gauge}, we have that 
$$
(\W_u \ast_u \D_t)\circ_t \V_{m,1}\cong \W_u\ast_u(\D_t \circ_t \V_{m,1}) \cong \W_u \ast_u \V_{m,1}\cong \V_{m+1,1}~,
$$
where we have used Lemma~\ref{lem:mix_ff_cap}.
Now, we proceed by induction on $n$. We have just established the base case for $n=1$ so suppose $n>1$ then
\begin{equation}\nonumber
\begin{split}
	\V_{1,1}\circ_t \V_{m,n} &\cong \V_{1,1}\circ_t (\V_{m+1,n-1}\circ_u \V_{1,1})~, \\
	&\cong (\V_{1,1}\circ_t \V_{m+1,n-1})\circ_u \V_{1,1} ~,\\
	&\cong \V_{m+2,n-1}\circ_u \V_{1,1}\, \\ 
	&\cong \V_{m+1,n}~,
\end{split}
\end{equation}
where in the second line we have used Lemma~\ref{lem:gauge_ut}.
\end{proof}

\begin{prop}\label{prop:gauge_mix}
Under gauging, the vertex algebras $\V_{m,1}$ behave as expected, namely
\begin{equation}\nonumber
\begin{split}
\V_{m,1}\circ_t \V_{p,q}&\cong \V_{m+p,q}~,\\
\V_{m,1}\circ_u\V_{p,q}&\cong \V_{p+m-2,q+1}~.
\end{split}
\end{equation}
\end{prop}
\begin{proof}
We proceed via induction for each type of gluing, noting that the base case $m=1$ is true, either by Lemma~\ref{lem:gauge_mix_trin} or by definition.

Suppose $m>1$, then
\begin{equation}\nonumber
\begin{split}
\V_{m,1}\circ_t\V_{p,q} &\cong (\V_{1,1}\circ_t\V_{m-1,1})\circ_t\V_{p,q}~,\\
&\cong \V_{1,1}\circ_t(\V_{m-1,1}\circ_t\V_{p,q})~,\\
&\cong \V_{p+m,q}~,
\end{split}
\end{equation}
where in the second line, we have used Lemma~\ref{lem:rearr_gauge} to arrive at the desired result.

Next we treat the $\circ_u$ case. Again, suppose $m>1$, then
\begin{equation}\nonumber
\begin{split}
\V_{m,1}\circ_u\V_{p,q} &\cong (\V_{1,1}\circ_t\V_{m-1,1})\circ_u\V_{p,q}~,\\
&\cong \V_{1,1}\circ_t(\V_{m-1,1}\circ_u\V_{p,q})~,\\
&\cong \V_{p+m-2,q+1}~,
\end{split}
\end{equation}
where, in the second line we have used a slight modification of Lemma~\ref{lem:gauge_ut} --- which applies, since the cohomology $\V_{1,1}\circ_t-$ is in degree zero so the spectral sequences will collapse at the second page.
\end{proof}

It is our belief that we should be able to extend these results to the general case
\begin{equation}
	\V_{m,n}\circ_t \V_{p,q} \cong \V_{m+p,n+q-1}~, \quad \V_{m,n}\circ_u \V_{p,q} \cong \V_{m+p-2,q+n}~.
\end{equation}
The obstructions are as follows.
In the case of $\circ_t$, the inductive step is $\V_{m,n}\circ_t(\V_{p+1,q-1}\circ_u \V_{1,1})$ and the corresponding spectral sequence is unbounded and does not collapse at the second page. Similarly for the untwisted gluing we cannot establish the putative isomorphism
\begin{equation}
	(\V_{1,1}\circ_u\V_{m+1,n-1})\circ_u\V_{p,q}\cong \V_{1,1}\circ_u(\V_{m+1,n-1})\circ_u\V_{p,q}~,
\end{equation}
for the inductive step.
Neither cohomology is concentrated in degree zero and so the second page of the spectral sequence is unbounded. To make progress, we need better machinery.

\begin{prop}~\label{prop:ff-untwisted-mixed}
We have the isomorphism
$$
\V_{G_u,s}\ast_u \V_{m,n} \cong \V_{m+s,n}~.
$$
\end{prop}
\begin{proof}
We proceed by induction on $s$, noting that, for $s=1$, the statement is true since $V_{m,n}$ are in $\KL_{u,0}$. Now suppose $s>1$, and consider $H^0_{DS}(u,\V_{G_u,s}\ast_u \V_{m,n})$. Of course, $H^0_{DS}(u,-)$ and $\W_u\circ_u -$ are isomorphic. We form the bicomplex 
$$
C^{\bullet, \bullet} = \W_{u}\otimes \V_{G_u,s} \otimes \V_{m,n}\otimes \Li{\bullet}(\zf(\gf_u)))\otimes \Li{\bullet}(\gf_u)~,
$$
with differentials $d_\zf$ acting on $\V_{G_u,s} \otimes \V_{m,n}\otimes \Li{\bullet}(\zf(\gf_u))$ and $d_{\gf}$ acting on $\W_u\otimes\V_{G_u,s}\otimes \Li{\bullet}(\gf_u)$. The differentials anticommute and we can form the total complex as usual. The two relevant spectral sequences are
\begin{equation}\nonumber
\begin{split}
_I E_{2}^{p,q} = \Hi{p}(\hat{\gf}_{u,-\kappa_g},\gf_u, \W_u \otimes \Hi{q}(\ZZ_u,\V_{G_u,s}\otimes \V_{m,n}))~,\\
_{II} E_{2}^{p,q} = \Hi{p}(\ZZ_u,\Hi{q}(\hat{\gf}_{u,-\kappa_g},\gf_u, \W_u\otimes \V_{G_u,s})\otimes \V_{m,n})~.
\end{split}	
\end{equation}
The functor of DS-reduction is exact and so both sequences collapse at page two with $_I E_{2}^{0,q}$ and $_{II}E_{2}^{p,0}$ being the only non-zero entries. This gives the isomorphism,
$$
H^0_{DS}(u,\V_{G_u,s}\ast_u\V_{m,n}) \cong \V_{G_u,s-1}\ast_u\V_{m,n} \cong \V_{m+s-1,n}~,
$$
where we used the inductive hypothesis. Acting by $\W_u\ast_u-$, we have that
\begin{equation}
	\V_{G_u,s} \ast_u \V_{m,n} \cong \V_{m+s,n}~,
\end{equation}
as desired.
\end{proof}

Finally, let us consider gauging the untwisted and mixed vertex algebras together.
\begin{prop}
Under untwisted gauging of untwisted vertex algebras, the mixed vertex algebras behave as expected,~\ie
$$
\V_{G_u,s} \circ_u \V_{m,n} \cong \V_{m+s-2,n}
$$
\end{prop}
\begin{proof}
We have the following chain of isomorphisms,
\begin{equation}\nonumber
\begin{split}
	\V_{G_u,s}\circ_u\V_{m,n} &\cong (\V_{G_u,s-1}\ast_u \W_u)\circ_u \V_{m,n} \,\\
	&\cong \V_{G_u,s-1} \ast_u (\W_{u}\circ_u \V_{m,n})~,\\
	&\cong \V_{G_u,s-1} \ast_u \V_{m-1,n}~,\\
	&\cong \V_{m+s-2,n}~,
\end{split}
\end{equation}
where in the second line we have used Lemma~\ref{lem:rearr_gauge_ff} and in the third we have used Proposition~\ref{prop:ff-untwisted-mixed}.
\end{proof}

The machinery of Feigin-Frenkel gluing has been invaluable to our proof of invariance under the $4$-move. Yet, in some sense it is an unnatural construction in that we must truncate to the zeroth cohomology by hand. The natural construction would involve some functor, which is exact in the genus-zero cases of Arakawa. In the twisted case, the higher derived functors would hopefully capture the fermions that arise from residual gauge symmetry in the genus-zero case. Unfortunately, we do not currently have a good candidate for such a functor.

To finish, we wish to address the issue of associativity. In~\cite{Arakawa:2018egx}, the cohomology $\V_{G,s}\circ\V_{G,s'}$ was concentrated in degree zero and so, by means of a spectral sequence argument, is associative. In our case, the argument is not so simple --- we have repeatedly remarked that zero genus is no longer sufficient for a gluing to be concentrated in degree zero. Our usual spectral sequence no longer collapses on the second page and so the proofs of our rearrangement lemmas no longer hold.
Nevertheless, it is our belief that associativity must still hold in general. Yanagida~\cite{Yanagida:2020kim} has provided a derived version of the construction of~\cite{Arakawa:2018egx}. In addition, they have also lifted the Moore--Tachikawa TQFT to the derived setting. In the derived Moore--Tachikawa setting, associativity of gauging follows from properties of the derived pushforward --- even in the nonzero genus case.
However, the notion of associativity in the derived setting is not quite what we mean by associativity. In short, we pass to cohomology before the second gauging --- unlike the derived case, where one does not pass to cohomology but instead holds on to the data of the complex. A sufficient condition for the derived associativity to imply our version of associativity is to show that the relevant chain complexes are formal,~\ie\ are isomorphic to their cohomology (thought of as a complex with zero differential) in the \textit{derived} category. While this is an interesting problem, we will not address it in this work.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\label{ssec:duality}Generalised \texorpdfstring{$S$}{S}-duality and 4-moves}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We will restrict ourselves to the sub-web of generalised $S$-dualities that can be reached by repeated application of the various $4$-moves. Assuming gauging is associative, this recovers a large swathe of the $S$-duality landscape. For the untwisted, genus zero, vertex algebras, the operation of gauging was shown to be associative in~\cite{Arakawa:2018egx}. 

Let $\V$ be some mixed vertex algebra, for now we assume genus zero with only maximal punctures. There are three different types of $4$-move that can act on $\V$. The first acts on a collection of four untwisted punctures; the second acts on two pairs of twisted punctures and the third acts on a pair of twisted punctures and two untwisted punctures. We shall examine each case, in turn, to establish invariance.

In the purely untwisted case, invariance under the $4$-move is baked into Arakawa's construction, which is manifestly permutation symmetric in the moment maps. Let us present an alternate formulation, which is generalisable to the twisted case. We may endow $V_{G,s}$ with the action\footnote{As written, the action of the $4$-move is not an automorphism but an isomorphism to some vertex algebra object in $\KL$. To correct this to an automorphism, we appeal to the uniqueness property of $\V_{G,s}$ (see Remark 10.13 of~\cite{Arakawa:2018egx}) and fix an isomorphism from this vertex algebra back to $\V_{G,s}$. One can perform a similar trick with $\V_{m,n}$ using the uniqueness statements of the previous section. To avoid having to make such a choice one can work with the Moore--Seiberg groupoid~\cite{Moore:1104178762} but we will not do so here.}
of a permutation group as follows. First, we close off the punctures labelled $2$ and $3$ in order,~\ie\ we perform DS reduction with respect to the moment maps $\iota_2$, associated to puncture $2$, and then with respect to $\iota_3$, associated to puncture $3$. We can invert this procedure by FF-gluing a cap with moment map $\iota_3$ and then FF-gluing a cap with moment map $\iota_2$. Instead, we reverse the order of inversions, that is to say we first glue a cap with moment map $\iota_2$ and then a cap with moment map $\iota_3$. This is an isomorphism since
%%%%%%
\begin{equation}
	\W_{G,3}\ast_u(\W_{G,2}\ast_u(\W_{G,3}\circ_u(\W_{G,2}\circ_u \V))) \cong \W_{G,2} \ast_u (\W_{G,3}\ast_u	(\W_{G,3}\circ_u(\W_{G,2}\circ_u \V)))\cong \V~,
\end{equation}
%%%%%%
where we have used Lemma~\ref{lem:rearr_ff} to swap the order of FF-gluings. The subscripts on the caps keep track of the labelling of the moment maps.
One can realise the actions of the other transpositions in the same way and thus generate the action of the full symmetric group on $s$ punctures. The action of the symmetric group should be understood as swapping the labellings of the moment maps associated to each puncture. This argument also establishes invariance under the four move, of the first type, for the mixed vertex algebras $\V_{m,n}$ too.

Now let us consider the case $\V=\V_{m,n}$, the mixed vertex algebra with two pairs of twisted punctures and no untwisted punctures. We can define the action of transpositions, as in the untwisted case, by closing pairs of punctures and gluing caps. Again, let us pick two twisted punctures, labelled $2$ and $3$, with moment maps $j_2$ and $j_3$ respectively. We perform $DS$ reduction once more, closing the punctures labelled $2$ and then $3$, in order. Once again, we restore the punctures by FF-gluing, via the twisted Feigin--Frenkel centre, two twisted caps with moment maps $j_2$ and $j_3$. We have 
\begin{equation}
	\W_{t,2}\ast_t (\W_{t,3}\ast_2(\W_{t,3}\circ_t(\W_{t,2}\circ_t \V))) \cong \W_{t,3}\ast_2(\W_{t,3}\ast_2(\W_{t,3}\circ_t(\W_{t,2}\circ_t \V)))\cong \V~.
\end{equation}
Once more, by Lemma~\ref{lem:rearr_ff}, this results in a vertex algebra that is isomorphic to $\V_{0,2}$. All transpositions of twisted punctures can be arrived at using this method and we can generate the full symmetric group on $2n$ twisted punctures. It should be noted that the automorphism group allows swaps between twisted punctures that are not connected by a twist line. For example, the automorphisms on $\V_{0,2}$ is not $\IZ_2\times \IZ_2$, which swaps punctures connected by twist lines, but the full $S_4$.

%Suppose $\V$ is some, possibly mixed, genus zero vertex algebra. Consider any collection of four punctures, all twisted or untwisted. By our previous arguments, the action of $S_4$ on such a collection results in a isomorphic vertex algebra. Thus we have invariance under the $4$-move of the first and second kind.

For the $4$-move of the third kind, our analysis in terms of permutation groups fails. This move swaps between the degeneration limits shown in Figure~\ref{fig:ut-move} --- unlike the other cases the decompositions are no longer related by a simple permutation on the punctures. Instead, we appeal to Proposition~\ref{prop:ff-untwisted-mixed} which states that the two BRST gluings $\V_{m-1,n}\circ_u\V_{G_u,3}$ and $\V_{1,1}\circ_t\V_{m-1,n}$ are isomorphic.

These $4$-moves, in addition to the assumption that $\circ_t$ and $\circ_u$ are always associative, recovers the entire landscape of generalised $S$-duality --- up to, of course, the $ab$-moves that appear at higher genus.

A proof of invariance under the $ab$-move eludes us but we shall pose this as a conjecture in the language of semi-infinite cohomology.
\begin{conj}
Let $\V_{G_u,3}$ be the trinion vertex algebra with maximal untwisted punctures and $\V_{1,1}$ be the mixed trinion vertex algebra as before. Let $i_1,i_2,i_3$ denote the three actions of $V^{\kappa_c}(\gf_u)$ on $\V_{G_u,3}$. Similarly, let $j_2,j_3$ be the actions of $V^{\kappa_c}(\gf_t)$ on $\V_{1,1}$.
Then we have the isomorphism
$$
\Hi{\bullet}(\hat{g}_{u,-\kappa_g},\gf_u,\V_{G_u,3})\cong \Hi{\bullet}(\hat{\gf}_{t,-\kappa_g},\gf_t,\V_{1,1})\,,
$$
where $\hat{\gf}_{u,-\kappa_g}$ acts on $\V_{G_u,3}$ via $i_2\otimes (i_3\circ \sigma)$, with $\sigma$ the $\IZ_2$ outer-automorphism, and $\hat{\gf}_{t,-\kappa_g}$ acts on $\V_{1,1}$ via $j_2\otimes j_3$.
\end{conj}

Establishing invariance under the $ab$-move for the one punctured torus is sufficient to ensure invariance for the vertex algebras of all other surfaces. This construction is explicitly at nonzero genus and so the higher cohomologies will be nonvanishing. We also wish to note that this one-punctured torus is not only of, purely, algebraic interest. The SCFT on the (minimal) one-punctured torus is an $\NN=4$ SYM theory with gauge algebra $\gf_u$ or $\gf_t$, depending on the cycle. In addition there are, decoupled, free hypermultiplets transforming with the flavour symmetry of the puncture, which come along for the ride under $S$-duality transformation. Thus, the conjecture we have made is very natural, from a physics perspective, and is motivated from generalised $S$-duality in $\NN=4$ theories.

While we are unable to show that the vertex algebras themselves are invariant under the $ab$ move, we are able to show that the Schur index is. Clearly from the form of (\ref{eq:indfull}), the index is invariant under any permutation of identical punctures and so is invariant under the $4$-move. To establish invariance under the $ab$-move all we have to show is that the indices of the one punctured tori agree. The index of an untwisted trinion with maximal punctures is
\begin{equation}
	\mathcal{I}(\mathbf{a},\mathbf{y},\mathbf{z}) = \sum_{\lambda\in P_{u}^+} \frac{\mathcal{K}_u(\mathbf{a})\chi^\lambda_u(\mathbf{a})\mathcal{K}_u(\mathbf{y})\chi^\lambda_u(\mathbf{y})\mathcal{K}_u(\mathbf{z})\chi^\lambda_u(\mathbf{z})}{\mathcal{K}_u(\times)\chi^\lambda_u(\times)}~.
\end{equation}
The gauging procedure is then
\begin{equation}
	\mathcal{I}_a(\mathbf{a}) = \oint [\mathrm{d}\mathbf{y}][\mathrm{d}\mathbf{z}]\Delta(\mathbf{y}) \mathcal{I}(\mathbf{a},\mathbf{y},\mathbf{z}) \mathcal{I}^V(\mathbf{y}) \delta(\mathbf{y},\sigma(\mathbf{z}^{-1}))~.
\end{equation}
Notice, that the usual propagator has been modified to $\delta(\mathbf{y}_1,\sigma(\mathbf{x}_2^{-1}))$ to account for the fact that the diagonal action has been twisted. Expanding the above expression, we have 
%%%%%%
\begin{equation}
\begin{split}
	\mathcal{I}_a(\mathbf{a}) &= \oint[\mathrm{d}\mathbf{z}]\Delta(\mathbf{z}) \mathcal{I}^V(\mathbf{z})\delta(\mathbf{y},\sigma(\mathbf{z}^{-1})) \sum_{\lambda\in P_u^+} \frac{ \mathcal{K}_{u}(\mathbf{y})\chi^{\lambda}_{u}(\mathbf{y})\mathcal{K}_{u}(\mathbf{z})\chi^{\lambda}_{u}(\mathbf{z})}{\mathcal{K}_{u}(\times)\chi^{\lambda}_{u}(\times)}~,\\
	&= \sum_{\lambda\in P_u^+}\frac{\oint[\mathrm{d}\mathbf{z}]\Delta(\mathbf{z}) \mathcal{I}^V(\mathbf{z}) \mathcal{K}_{u}(\mathbf{z})\mathcal{K}_{u}(\sigma(\mathbf{z})^{-1})\chi^{\lambda}_{u}(o(\mathbf{z}^{-1}))\chi^{\lambda}_{u}(\mathbf{z})}{\mathcal{K}_{u}(\times)\chi^{\lambda}_{u}(\times)}~,\\
	&= \sum_{\lambda\in P_u^+}\frac{\oint[\mathrm{d}\mathbf{z}]\Delta(\mathbf{z}) \mathcal{I}^V(\mathbf{z}) \mathcal{K}_{u}(\mathbf{z})\mathcal{K}_{u}(\mathbf{z}^{-1})\chi^{\sigma(\lambda)}_{u}(\mathbf{z}^{-1}))\chi^{\lambda}_{u}(\mathbf{z})}{\mathcal{K}_{u}(\times)\chi^{\lambda}_{u}(\times)}~,
	\end{split}
\end{equation}
%%%%%%
where in the third line, we have used the transformation property of the group characters to move the outer automorphism to the Dynkin label. The orthonormality property of characters restricts the sum to only those weights $\lambda\in P_u^+$ that are invariant under $\sigma$. This is equivalent to summing over $P_t^+$ and so, by our usual abuse of notation, we have
%%%%%%
\begin{equation}
	\mathcal{I}_a(\mathbf{a}) = \sum_{\lambda\in P_t^+}\frac{\mathcal{K}_u(\mathbf{a})\chi^\lambda_u(\mathbf{a})}{\mathcal{K}_u(\times)\chi^\lambda_u(\times)}~.
\end{equation}
%%%%%%
The index of $\CC_{0,1,1}$ is 
%%%%%%
\begin{equation}
	\II_{\CC_{0,1,1}}(\mathbf{a},\mathbf{b}_1,\mathbf{b}_2) = \sum_{\lambda\in P_t^+} \frac{\KK_u(\mathbf{a})\chi_u^\lambda(\mathbf{a})\KK_t(\mathbf{b}_1)\chi_t^\lambda(\mathbf{b}_1) \KK_t(\mathbf{b}_2)\chi_t^\lambda(\mathbf{b}_2)}{\KK_u(\times)\chi_u^\lambda(\times)}.
\end{equation}
%%%%%%
Gauging the diagonal $\gf_t$ action on $\CC_{0,1,1}$ results in the character:
%%%%%%
\begin{equation}
	\II_b(\mathbf{a}) = \oint[\mathrm{d}\mathbf{b}_1] \II_{\CC_{0,1,1}}(\mathbf{a},\mathbf{b}_1,\mathbf{b}_2)\II^V(\mathbf{b}_1)\delta(\mathbf{b}_2,\mathbf{b}_1^{-1})~,
\end{equation}
%%%%%%
where the contour integral is over the maximal torus of the twisted algebra. It is straightforward to see that $\II_a(\mathbf{a})=\II_b(\mathbf{a})$, as expected.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\label{ssec:z3-twist}The \texorpdfstring{$\IZ_3$}{Z3} twist of \texorpdfstring{$\df_4$}{d4}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We have avoided addressing the $\IZ_3$ twist, since we believe it requires genuinely new technology compared to the $\IZ_2$ case. With a $\IZ_3$ twist, there is the possibility of a trinion with three twisted punctures, all with a monodromy of $\omega\in\IZ_3$ or its inverse $\omega^2$.
Much like the $\IZ_2$ case has fermions at genus zero, we will argue that the $\IZ_3$ case has fermions appearing at three puncture.
Nevertheless, we can still make some statements on the $S$-duality properties of the $\IZ_3$ mixed vertex algebras.

The chiral differential operators over $G_2$ are well defined. Here we take $G_2$ to be the exponentiated form of the $\gf_2$ Lie algebra, \ie~$G_2$ is a simply connected, semi-simple, algebraic Lie group. The superconformal index assigned to the twisted cylinder agrees with the character of $\V_{G_2,2}$ and this shall once more motivate our construction.

Pictorially, one imagines the cylinder as having a puncture twisted by $\omega$ and the other by $\omega^2$. One might therefore, \textit{a priori}, expect that there are two possible $\gf_2$ caps, $\W_\omega$ and $\W_{\omega^2}$, depending on which puncture is closed. Yet, from the uniqueness argument of~\cite{Arakawa:2018egx}, both caps must be isomorphic. The outer-automorphism, $\sigma$, should, therefore, lift to an isomorphism of vertex-algebras $\W_{\omega}\xrightarrow{\sigma}\W_{\omega^2}$. We define the mixed trinion, $\V_{1,1}$ as
%%%%%%
\begin{equation}
	\V_{1,1} \coloneqq \W_u\ast\D_{G_2}~.
\end{equation}
%%%%%%
Examining the list of fixtures from~\cite{Chacaltana:2016shw}, we see that no mixed trinion theory (with typical punctures) is free.

The total monodromy around all punctures must be trivial. Thus, surfaces must have twist lines starting on a puncture $\omega$ and ending on a puncture labelled $\omega^2$. Once again, we denote a genus zero surface with $m$ untwisted punctures and $n$ $\omega,\omega^2$ pairs of punctures by $\CC_{0,m,n}$. The genus zero vertex algebras are once more denoted by $\V_{m,n}$ and are constructed as before. The ambiguity in the two versions of the cap is present here again. If one were to swap two punctures with $\omega$ and $\omega^2$ labels, is the resulting vertex algebra still isomorphic to the original? We believe the answer is yes.

Let us first establish some rearrangement lemmas for the $\IZ_3$ case. The isomorphism of vertex algebras $\W_\omega\cong\W_{\omega^2}$ lifts to a natural isomorphism of functors
%%%%%%
\begin{equation}
	\Hi{0}(\ZZ_t,\W_\omega\otimes-) \simeq \Hi{0}(\ZZ_t,\W_{\omega^2}\otimes-)~.
\end{equation}
%%%%%%
Though unphysical, one can consider the vertex algebra $\widetilde{\V}_{1,1}\coloneqq \W_\omega\ast_t(\W_\omega\ast_u\W_u)$. This would correspond to the surface with two maximal punctures twisted by $\omega$ and an untwisted puncture.
From the natural isomorphism, however, we have that
%%%%%%
\begin{equation}
	\widetilde{\V}_{1,1}\cong \V_{1,1}~.
\end{equation}
%%%%%%
We can, therefore, use the trinion $\widetilde{\V}_{1,1}$ as the building block for an equivalent construction of genus zero vertex algebras, which are isomorphic to the construction with respect to $\V_{1,1}$. This construction, however, makes manifest the enhanced symmetry of the vertex algebras, \ie~the labelling by $\omega,\omega^2$ is redundant. 

Let us reiterate, since it is a surprising result. The genus zero mixed vertex algebras are uniquely specified (up to isomorphism) by the number of maximal untwisted punctures and the number of pairs of maximal twisted punctures. This has interesting consequences for generalised $S$-duality --- the $4$-move can swap $\omega$ and $\omega^2$ punctures. For example, the naive symmetry of $\CC_{0,0,2}$ is $\IZ_2\times\IZ_2$, which swaps the punctures with the same label, but this is enhanced to $S_4$ --- swapping between all four punctures. 
In general the action of $4$-moves on $\V_{m,n}$ generates the permutation group $S_{2n}$ instead of $S_n\times S_n$. 

In addition to the mixed trinion that we have described there, one can compactify on a curve with a three pronged twist line --- connecting three punctures with an $\omega$ (or $\omega^2$) twist.
The trinion with three $\omega$ punctures does indeed correspond to a physical SCFT. One might expect that this trinion is $\V_{G_2,3}$. Comparing the superconformal index of this trinion theory with the character of $\V_{G_2,3}$, however, shows that this cannot be the case. Indeed, this trinion is something of a mystery and we currently have no way of constructing it with the machinery of~\cite{Arakawa:2018egx}. For now, we shall refer to the surface with the three pronged twist line by $\CC_{0,0,3\omega}$ and its corresponding vertex algebra by $\V_{0,3\omega}$. We also introduce their $\sigma$-conjugates $\CC_{0,0,3\omega^2}$ and $\V_{0,3\omega^2}$, which correspond to the surface with a three pronged twist line between three $\omega^2$ twisted punctures and its associated vertex algebra. It is tempting to posit the duality $\V_{0,3\omega}\cong \V_{0,3\omega^2}$, but since we have no construction of these vertex algebras nothing precise can be said.

Unlike all of the other trinions we have considered, we believe $\V_{0,3\omega}$ contains fermions, in the sense that $\V_{0,3\omega}$ has a cohomological grading in which it is not concentrated in degree zero. Any construction invloving FF gluing is forced to be in degree zero, since we manually truncate to the zeroth cohomology. It is perhaps here where a new form of FF-gluing shall shed some light. 

%In light of our discussion on the effective genus, we propose that this surface has effective genus greater than zero. Equivalently, the associated vertex algebra should contain fermions. This would go some way in explaining why the construction is elusive. Any construction involving FF-gluing or BRST gauging of $G_2$ caps  will be concentrated in degree zero. We, therefore, require new technology in order to construct this vertex algebra. 

Let us provide some motivation for our belief: the SCFT associated to $\CC_{0,0,3\omega}$ participates in the following $S$-duality~\cite{Chacaltana:2016shw}, involving the $D_4-G_2$ mixed trinion, $\CC_{0,1,1}$. We have that 
%%%%%%
\begin{equation}
	\CC_{0,1,1}\circ_u\CC_{0,1,1} \cong \CC_{0,0,3\omega}\circ_t\CC_{0,0,3\omega^2}~,
\end{equation}
%%%%%%
where the compositions, $\circ_u$ and $\circ_t$, should be understood as BRST gauging operations on the associated SCFTs. The gluing on the left hand side is between the punctures labelled by $\omega$ and $\omega^2$. From our discussions on the free-cofree property of the mixed trinion we believe that $\V_{1,1}\circ_u\V_{1,1}$ is not concentrated in degree zero and so contains fermions. Thus, the gluing, $\V_{0,3\omega}\circ_t\V_{0,3\omega^2}$, must contain fermions. There are two (not mutually exclusive) possibilities: the vertex algebra $\V_{0,3\omega}$ and its $\sigma$-conjugate already contain fermions which survive the gluing; alternatively, the vertex algebra $\V_{0,3\omega}$ does not satisfy the free-cofree property. 
In either case, we cannot reproduce these properties starting from $\D_t$, $\W_t$ and the operations of FF-gluing and gauging. All such gluings have vanishing negative cohomology and so cannot reproduce the desired fermions. It is, perhaps, here that a modified version of FF-gluing will come into play. 


